No-regret Algorithms for Fair Resource Allocation

We consider a fair resource allocation problem in the no-regret setting against an unrestricted adversary. The objective is to allocate resources equitably among several agents in an online fashion so that the difference of the aggregate $\alpha$-fair utilities of the agents between an optimal static clairvoyant allocation and that of the online policy grows sub-linearly with time. The problem is challenging due to the non-additive nature of the $\alpha$-fairness function. Previously, it was shown that no online policy can exist for this problem with a sublinear standard regret. In this paper, we propose an efficient online resource allocation policy, called Online Proportional Fair (OPF), that achieves $c_\alpha$-approximate sublinear regret with the approximation factor $c_\alpha=(1-\alpha)^{-(1-\alpha)}\leq 1.445,$ for $0\leq \alpha < 1$. The upper bound to the $c_\alpha$-regret for this problem exhibits a surprising phase transition phenomenon. The regret bound changes from a power-law to a constant at the critical exponent $\alpha=\frac{1}{2}.$ As a corollary, our result also resolves an open problem raised by Even-Dar et al. [2009] on designing an efficient no-regret policy for the online job scheduling problem in certain parameter regimes. The proof of our results introduces new algorithmic and analytical techniques, including greedy estimation of the future gradients for non-additive global reward functions and bootstrapping adaptive regret bounds, which may be of independent interest.

==> analysis.tex <==
\section{System Model for the Caching Problem} \label{formulation}
We consider an online problem, which we call \emph{Online Fair Caching} (OFC). In this problem, $m$ users are connected to a single cache of capacity $k$ (see Figure \ref{sys-diagram} for a schematic). At each round, every user request one file from a library of size $N.$ The file request sequence could be adversarial. At the beginning of each round $t$, an online caching policy prefetches $k$ files on the cache, denoted by the vector $y_t \in \{0,1\}^N$ such that $||y_t||_1=k.$ The set of all feasible caching configuration is denoted by $\Delta^N_k.$ 
\footnote{In the following, we consider the relaxed action where the components of any vector $y \in \Delta^N_k$ denote the corresponding inclusion probabilities. From the any relaxed action, one can derive an integral caching policy by using Madow's sampling with these probabilities. As a result, the variable $R_i(t)$'s in the regret definition are to be taken as the expected hit rates (\emph{not} the actual hits), which can be computed by the policy from the inclusion probabilities $\bm{y}_t$ as in Eqn.\ \eqref{reward-evolution}.}.  Immediately after the prefetching at round $t$, each user $i$ reveals its file request, represented by the one-hot encoded vector $x_i(t)$, $1\leq i \leq m$. A special case of the above caching model for a single user ($m=1$) has been investigated in our previous work \citep{SIGMETRICS20, paria2021, mhaisen2022optimistic, ITW22}. 

\begin{figure}[!ht]
\centering
	\includegraphics[scale=0.3]{diagram.pdf}
	\put(-35, 35){Library}
	\put(-155,35){Cache of capacity $k$}
	\put(-265,99){User $1$}
    \put(-265,64){User $2$}
    \put(-268,10){User $m$}
	\caption{System model}
	\label{sys-diagram}
\end{figure}

Let the variable $R_i(t)$ denote the cumulative hits obtained by the $i$\textsuperscript{th} user up to round $t \geq 1$. Clearly,
\begin{eqnarray} \label{reward-evolution}
	R_i(t+1) = R_i(t) + \langle x_i(t), y_t \rangle, ~~1 \leq i \leq m,
\end{eqnarray}
where $R_i(0)=0, \forall i. $ By iterating the above recursion, the variable $R_i(t)$ can be alternatively expressed as follows:
\begin{eqnarray} \label{hit-eqn}
	R_i(t) = \sum_{\tau=1}^t \langle x_i(\tau), y_\tau \rangle.
\end{eqnarray}
From the above, we can see that $R_i(t)$ is a function of only the first $t$ caching action variables $\{y_\tau\}_{\tau=1}^t.$ Let the utility function for any user be given by the concave function $\phi: \mathbb{R}_+ \to \mathbb{R}_+,$ where the function $\phi$ belongs to the class of all admissible utilities defined later. In the sequel, we will exclusively work with the $\alpha$-fair utility function 
\begin{eqnarray} \label{alpha-fair}
	\phi(x)=\phi_\alpha(x)\equiv  w_\alpha\frac{x^{1-\alpha}}{1-\alpha}, ~~x\geq 0,
\end{eqnarray}
for some constant $w_\alpha \geq 0$ and $0\leq \alpha <1.$
Our objective is to design an online caching policy that minimizes the regret corresponding to the aggregate utilities of all users at round $T,$ compared to any offline time-invariant caching-configuration that caches a fixed set of $k$ files $y^*$ at all rounds $t \in [T]$. Assume that the static benchmark configuration yields a cumulative cache hit vector of $\bm{R}^*(T)$ on round $T.$ For some small fixed constant $c\geq 1,$ our objective is to design a caching policy which minimizes the $c$-regret defined as follows:
\begin{eqnarray} \label{regret-def}
	\min_{\{y_t\}_{t=1}^T}\mathcal{R}_T \equiv \sum_{i=1}^m \phi(R_i^*(T))-   c\sum_{i=1}^m \phi(R_i(T)),
\end{eqnarray}
for all $T \geq 1$. The horizon length $T$ is not necessarily known to the policy a priori. 
In the special case when $\alpha =1, c=1$ the above problem reduces to the problem of minimizing regret for cumulative hits \citep{SIGMETRICS20}.
We emphasize that, although the benchmark policy $y^*$ remains fixed, the cumulative hit rates $R_i^*(t)$ vary with time according to the adversarial dynamics \eqref{reward-evolution}.
% Similar utility function-based performance optimization for networks has been considered earlier in stochastic setting \citep{andrews2005optimal}.
\iffalse
\subsection{Admissible utility functions}
In practice, there could be a range of choices for the utility (also known as \emph{fairness}) function $\phi$ \footnote{Our results can be straight-forwardly generalized to time-varying utility functions $\phi_t(\cdot)$ as well.}. The utility functions could be application-specific, and most importantly, they could be \emph{transparent} to the online learner \emph{throughout} the entire time-horizon. In particular, no feedback might be available to the learner regarding its functional form or even its gradients. This should be contrasted with the usual Online Convex Optimization (OCO) framework \citep{zinkevich2003online}, where the gradient of the reward functions are revealed to the learner at the end of each round. The issue of learner not knowing the the utility function may arise from the fact that the true utility of the users may depend on the nature of the files being cached (\emph{e.g.,} whether the files contain movies or fixed datasets, or real-time data of a UAV). Furthermore, it could also be difficult to analytically characterize the true utility function. Interestingly, our proposed caching policy achieves a sublinear regret bound \emph{uniformly} for \emph{any} utility function in the class $\Phi$ up to determining a scalar hyper-parameter $0<\epsilon<1$ described later. 
%An interesting consequence of the above simple derivation is that the proposed policy $\pi$ continues to yield a sublinear regret if the utility functions satisfy some mild conditions.
%Assume that the fairness function of the $i$\textsuperscript{th} user at round $t$ be given by $\phi_i(t).$ Then, following the same line of derivation leading to \eqref{first-order-bound}, the regret, in this case, can be upper-bounded as:
%
%We now make the following assumptions on the class $\Phi$ of admissible utility functions.
We now characterize the class of all admissible utility functions in the following definition.  
\begin{framed}
\begin{definition}[(The class of admissible utility functions $\Phi$)] \label{admissible}
	The class of admissible utility functions  $\Phi$ consists of all functions $\phi : \mathbb{R}_+ \to \mathbb{R}_+$ satisfying the following two conditions:
	
	1. 	Each function $\phi \in \Phi$ is non-decreasing, differentiable, and concave.
	
	2. $J_\phi(T)\equiv \int_{0}^T \sqrt{x} \phi'(x) dx = o(T), \forall \phi \in \Phi.$
\end{definition}
\end{framed}
%\begin{assumption}
%
%\end{assumption}
%	%\item  for each user $i \in [m]$.
%	\begin{assumption}
%			$J(T)\equiv \int_{1}^T \sqrt{x} \phi_i'(x) dx = o(T).$
%	\end{assumption}
% 
%\end{enumerate}
%\end{framed}
Upon integrating by parts, Condition 2 can also be given an alternative characterization. Note that
\begin{eqnarray*}
	\int_1^T \sqrt{x} \phi'(x) dx = \sqrt{T}\phi(T) - \frac{1}{2}\int_{1}^T \frac{\phi(x)}{\sqrt{x}} dx.    
\end{eqnarray*}

Thus Condition 2 is equivalent to the following condition:
\begin{eqnarray*}
	\overline{g(T)} \geq  2 g(T)- o(1),
\end{eqnarray*}
where $g(x) \equiv \frac{\phi(x)}{\sqrt{x}},$ and the term on the left denotes the average value of the function $g$ in the interval $[0,T].$ 

\textbf{Examples:}  Many common utility functions used in practice are included in the admissible class $\Phi.$ This includes the logarithmic utility function $\phi_{\textrm{logarithmic}}(x)=\log(x)$, and $\alpha$-fair utility functions  $\phi_\alpha(x) = \frac{x^{1-\alpha}}{1-\alpha}$, where $\nicefrac{1}{2}<\alpha \leq 1.$ The integral $J_\phi(\cdot)$ for these classes of functions can also be easily evaluated in closed-form. 

%\subsubsection*{Closed-form expressions of the integral $J (\cdot)$ for common utility functions}
%\textbf{Case 1: Logarithmic Utility}

1. In the case of the logarithmic utility function, we have $\phi_{\textrm{logarithmic}}(x) = \log (x). $ Hence, 
\begin{eqnarray} \label{log-J}
	J_{\textrm{logarithmic}}(T) = \int_{0}^T \frac{\sqrt{x}}{x} dx = 2T^{\nicefrac{1}{2}},   
\end{eqnarray}
 which can be seen to be sublinear. 
 
 2. In the case of $\alpha$-fair utility, we have $\phi_\alpha(x)= \frac{x^{1-\alpha}}{1-\alpha},$ for some $0<\alpha<1.$ Hence,
 \begin{eqnarray} \label{J-alpha}
 	J_{\alpha-\textrm{fair}}(T) = \int_{0}^T \sqrt{x} \frac{1}{x^\alpha} dx = \frac{1}{3/2-\alpha}T^{3/2 - \alpha}.
 \end{eqnarray}
 It can be seen from the above expression that $J_\alpha(T)$ is sublinear as long as $\frac{1}{2}<\alpha <1.$
 

%\textbf{Note:} 1. The above result holds even for a sequence of time-varying utility functions $\{\phi_t()\}_{t \geq 1}$ satisfying the conditions. 

To recap, the Online Fair Caching problem has the following information structure- (1) The utility function $\phi \in \Phi$ remains unknown to the learner throughout. (2) The file requests $x_i(t), i \in [m]$ for round $t$ is revealed to the learner only after the caching decision $y_t \in \Delta^N_k$ is made for round $t$.   
\fi

\subsection{On the non-triviality of the \texttt{OFC} problem}

We now outline the fundamental difference between the OFC problem \eqref{regret-def} and the usual Online Convex Optimization (OCO) problem \citep{hazan2019introduction}. In the standard OCO problem, the reward accrued at any round $t$ depends on the action taken on round $t$ \emph{only}. In particular, the OCO framework applies to the  \emph{memoryless} systems where the action taken at a round does not affect the reward functions seen in the subsequent rounds. On the other hand, in the OFC problem, the caching action $\bm{y}_t \in \Delta^N_k$ taken at round $t$ affects \emph{all} future rewards through the cumulative hit vector $\bm{R}(t)$. For the same reason, recent online algorithms developed for systems with \emph{bounded memory} \citep{anava2015online} do not apply to the \textsf{OFC} problem. From a high-level perspective, the online fair caching problem is an instance of an adversarial Reinforcement Learning problem, for which no general algorithmic methodology is known. One of the main surprises of this paper is that the OFC problem can be essentially reduced to an instance of an OCO problem with a carefully defined sequence of reward functions.


%subroutines with \emph{perturbed} requests even when the utility functions are unknown. 
\iffalse
\section{Preliminaries} \label{prelims}
In this section, we recall some recent adaptive regret bounds achieved by OGD-like algorithms. The $L_p$-deviation of a sequence of reward function $\{f_t\}_{t=1}^T$ is defined as
\begin{eqnarray*}
	D_p= \sum_{t=1}^T \max_{x \in X} || \nabla f_t(x) - \nabla f_{t-1}(x)||_p^2. 
\end{eqnarray*}
The paper \cite{chiang2012online} proves the following static regret bound for the OEGD algorithm proposed in that paper:
\begin{theorem}[\cite{chiang2012online}] \label{adaptive-regret}
	When the $L_2$-deviation of the loss function is $D_2$, the regret of the OEGD algorithm is at most $O(\sqrt{D_2}).$
\end{theorem}
\fi

\section{Design of a no-regret policy} \label{analysis}
The central idea behind the design of our online policy is to reduce the \textsf{OFC} problem with memory to an instance of online linear optimization problem \emph{without memory}.
%, which can be solved with the standard OCO techniques \citep{SIGMETRICS20, mukhopadhyay2022k}. 
%In doing so, it turns out that one also needs to slightly perturb the input request sequence itself to make the reduction work.

Towards this end, fix some constant $\beta \geq 1,$ to be determined later.
Using the fact that $\phi(R_i(T))$ is a concave function of the previous action variables $\{y_{\tau}\}_{\tau=1}^T,$ using the first-order Taylor series bound for concave functions between the points $\{y^*\}_{t=1}^T$ and $\{\beta y_t\}_{t=1}^T$, we can write 
\begin{eqnarray} \label{first-order-bound}
\phi(R_i^*(T))- \beta^{1-\alpha}\phi(R_i(T))
&\stackrel{(a)}{=}&	\phi(R_i^*(T)) - \phi(\beta R_i(T)) \nonumber, \\
&\leq&  \beta^{-\alpha}\phi'(R_i(T)) \sum_{t=1}^T \langle x_i(t), y^*-\beta y_t \rangle.  
\end{eqnarray}
where in (a), we have used the explicit form of the $\alpha$-fair utility function that yields
\[ \phi(\beta x) = \beta^{1-\alpha} \phi(x), ~~\phi'(\beta x) = \beta^{-\alpha} \phi'(x).\]
In (a), we have also exploited the linearity of the cumulative hits $\bm{R}(T)$ w.r.t. the action variables $\{y_t\}_{t=1}^T$ from \eqref{hit-eqn} to conclude that scaling all action variables by a factor $\beta$ scales the cumulative hits by the same factor.  

Summing up the above inequality, we obtain the following upper bound for the $\beta^{1-\alpha}$-Regret of any online caching policy:  
\begin{eqnarray} \label{regret-expr3}
	\beta^{1-\alpha}-\textrm{Regret}_T \equiv \beta^{-\alpha}\sum_{t=1}^T \bigg( \langle \sum_{i} \phi'(R_i(T)) x_i(t), y^*-\beta y_t \rangle \bigg).
\end{eqnarray}

Note that the quantity $\phi'(R_i(T))$ depends on the entire sequence of actions $\{y_t\}_{t=1}^T.$ As such, \eqref{regret-expr3} is not a standard OCO problem as the value of $\phi'(R_i(T))$ is not known to the policy at any prior rounds $1\leq t\leq T$ and depends on its future actions and requests. To get around this fundamental issue, we now define a \emph{surrogate} online learning problem by replacing the term $\phi'(R_i(T))$ by its \emph{causal version} $\phi'(R_i(t))$ on round $t$. 
%and setting $\beta=1,$
In other words, we seek to design an online learning policy $\pi$ that minimizes the regret for the following Online Linear Optimization (OLO) problem:
 \begin{eqnarray} \label{surr-regret}
 	\hat{\textrm{Regret}_T} \equiv  \sum_{t=1}^T \bigg( \langle \sum_{i}\phi'(R_i(t)) x_i(t), y^*- y_t \rangle \bigg).
 \end{eqnarray}
To recapitulate the information structure, note that the cumulative hit vector $\bm{R}(t)$ is known, but the current request vector $\bm{x}(t)$ is unknown to the online learner before it makes caching decision $y_t.$ on the $t$\textsuperscript{th} round. 
  
We now make the following claim which is central to the design and analysis of our policy: 
\begin{framed}
\begin{theorem} \label{regret-comp}
Consider any arbitrary online caching policy $\pi$ and assume that the utility function of each user is given by the $\alpha$-fair utility function \eqref{alpha-fair}. Then, for any fixed benchmark caching configuration $y^*$, we have
\begin{eqnarray} \label{regret-comp-eq}
	c_\alpha-\textrm{Regret}_T \leq (1-\alpha)^{\alpha}\hat{\textrm{Regret}_T},
\end{eqnarray}
 where $c_\alpha \equiv (1-\alpha)^{-(1-\alpha)} \leq e^{1/e}<1.445.$
\end{theorem}
\end{framed}
\begin{proof}
%It is sufficient to consider the case when the $c_\alpha-\textrm{Regret}_T$ in the LHS of \eqref{regret-comp-eq} is non-negative. In case the $c_\alpha-\textrm{Regret}_T$ is negative for some benchmark $y^*$, there is nothing to prove.

The expression for $\beta^{1-\alpha}-\textrm{Regret}_T$ from Eqn.\ \eqref{regret-expr3} can be split into two terms as follows:
	\begin{eqnarray*}
		\beta^{1-\alpha}-\textrm{Regret}_T =\beta^{-\alpha}\big[\underbrace{\sum_i \phi'(R_i(T)) \sum_{t=1}^T \langle x_i(t), y^* \rangle}_{\textrm{\textcolor{blue}{$(A)$}}} - \beta \underbrace{\sum_i \phi'(R_i(T)) \sum_{t=1}^T \langle x_i(t), y_t \rangle}_{\textrm{\textcolor{blue}{$(B)$}}}\big].  
	\end{eqnarray*}
	Also denote the corresponding terms in the Regret expression \eqref{surr-regret} for the surrogate learning problem by $(A')$ and $(B')$. 
	We will now separately bound each of the above two terms in terms of the corresponding terms in the regret expression \eqref{surr-regret} for the surrogate learning problem. 
	
	\paragraph{\underline{Proving \textcolor{blue}{$(A)\leq (A')$}}}
	Recall that the utility function $\phi(\cdot)$ is concave. Hence, its derivative is non-decreasing in its argument. Furthermore, under the action of any policy, the cumulative hit $R_i(\cdot)$ is non-decreasing for each user $i \in [m].$ Thus, we have $\phi'(R_i(t)) \geq \phi'(R_i(T))$ for all $t \in [T], i\in [m].$ Hence, 
	\begin{eqnarray} \label{bd1}
	 (A) \leq \sum_{t=1}^T \langle \sum_i \phi'(R_i(t))x_i(t), y^*\rangle \leq (A'). 
	\end{eqnarray}
	
	\paragraph{\underline{Proving \textcolor{blue}{$(B') \leq (1-\alpha)^{-1}(B)$}}}
	We have 
	\begin{eqnarray} \label{bd2}
		(B)'&=& \sum_{i} \sum_{t=1}^T \phi'(R_i(t)) \langle  x_i(t), y_t \rangle \nonumber\\
		&=& \sum_i \sum_{t=1}^T \phi'(R_i(t)) \big(R_i(t+1)-R_i(t)\big) \nonumber\\
		&\leq & \sum_i \int_{0}^{R_i(T)} \phi'(R) dR \nonumber\\
		&=& \sum_i \phi (R_i(T))\nonumber\\
		&\stackrel{(a)}{=}& (1-\alpha)^{-1}\sum_i \phi'(R_i(T)) R_i(T)\nonumber\\
		&\stackrel{(b)}{=}& (1-\alpha)^{-1} \sum_i \phi'(R_i(T)) \sum_{t=1}^T \langle x_i(t), y_t\rangle  \nonumber\\
		&=& (1-\alpha)^{-1}(B),
	\end{eqnarray}
	where, in (a), we have used the explicit form of the $\alpha$-fair utility function to conclude that $x \phi'(x) = (1-\alpha)\phi(x)$\footnote{Strictly speaking, an upper-bound for (a) would have sufficed. }
 and in (b), we have used \eqref{hit-eqn}. Combining \eqref{bd1} and \eqref{bd2} and choosing $\beta= (1-\alpha)^{-1},$ we conclude that 
 \begin{eqnarray*}
 	(1-\alpha)^{-(1-\alpha)}-\textrm{Regret}_T \leq (1-\alpha)^\alpha \hat{\textrm{Regret}_T}. 
 \end{eqnarray*}
% Finally, since $\max_{0\leq \alpha <1}(1-\alpha)^{-(1-\alpha)}= e^{1/e},$ the result follows. 
\end{proof}
%\textbf{P.S.} Recall that, we dropped a scaling factor of $\beta^{-\alpha}$ in \eqref{regret-expr3}. With the choice of $\beta= (1-\alpha)^{-1}$, the RHS of Eqn.\ \eqref{regret-comp-eq} should be multiplied by a factor of  
\textbf{P.S.} Note that the scaling factor on the RHS with respect to the original regret is $\beta^{-\alpha}\leq 1.$ Hence, the above conclusion holds even without scaling as well. 



  \begin{algorithm}
\caption{Online Proportional Fair Caching (\texttt{OPFC})}
\label{OPFC}
\begin{algorithmic}[1]
\State \algorithmicrequire{ Fairness parameter $0\leq \alpha<1.$} Online file request sequence $\{x_i(t)\}_{t=1}^T$ from user $i, i \in [m],$ Euclidean projection oracle $\Pi_{\Delta^N_k}(\cdot)$ onto the feasible convex set $\Delta^N_k.$
\State \algorithmicensure{ Sequence of file inclusion probabilities $\{y_t\}_{t=1}^T$ and samples from this distribution}
\State $R_i \gets 1, \forall i\in [m], \bm{y}\gets \frac{k}{N}\mathds{1}_{N}, S\gets 0.$ \algorithmiccomment{\textcolor{black}{\emph{Initialization}}}
\ForEach {round $t=2:T$:}
\State $g \gets \sum_{i=1}^m \frac{x_i(t-1)}{R_i^\alpha}$ \algorithmiccomment{\emph{Computing the gradient}}
\State $S \gets S+ ||g||_2^2,$   \algorithmiccomment{\emph{Accumulating the norm of the gradients}}
\State $y \gets \Pi_{\Delta^N_k}\big(y+ \frac{k}{\sqrt{S}} g\big)$ \algorithmiccomment{\textcolor{black}{\emph{Updating the inclusion probabilities using OGA}}}
\State The users reveal their latest file requests $\{x_i(t), i \in [m]\}.$
\State $R_i \gets R_i + \langle x_i(t), y \rangle, ~\forall i\in [m].$ \algorithmiccomment{\textcolor{black}{\emph{Updating cumulative hits}}}
\State Cache file $S_t \gets \textsc{Madow-Sample}(y)$
%$k$ files according to the inclusion probability vector $y$ using Madow's sampling scheme described in Algorithm \ref{madow}
%given in Algorithm \ref{uneq} 
\algorithmiccomment{\textcolor{black}{\emph{Sample a subset of $k$ files by invoking Algorithm \ref{Madow}}}}
%according to the \textsc{FTRL}($\eta$) update 
%\eqref{ftrl-opt}. 
%\STATE Feed the vector $\bm{g}_t$ as the reward vector for round $t$ to the \textsc{FTRL} policy 
\EndForEach
\end{algorithmic}
\end{algorithm}


\iffalse

\section{Design of a No-regret Policy}
Assume that the cache capacity $k$ is no less than the number of users $m$ in the system. In this setup, we now design a no-regret policy for the logarithmic utility function against a much stronger comparator sequence $\pi^*=\{y^*_\tau\}_{\tau \geq 1}$ which, at each round $t$, caches all files requested by the users, \emph{i.e.,} $y^*_\tau = \bigvee_{i} x_i(\tau),$ where the $\bigvee$ operation is applied component wise. Clearly, the offline policy $\pi^*$ achieves the maximum utility over a time horizon, with $R_i(t) =t, \forall i,t.$ This yields the following optimal value for the offline cumulative utility function: 
\begin{eqnarray*}
	\textsc{Obj}^* = m \sum_{t=1}^T \log t \stackrel{\textrm{(Stirling)}}{\approx} m \bigg(\frac{1}{2}\log(2\pi T) + T \ln T -T \bigg) \approx mT\ln T.    
\end{eqnarray*}
We now design an online policy that achieves a sublinear regret with respect to this benchmark. Adapting the regret bound \eqref{regret-expr3} to the setting of time-varying benchmark, we have 
\begin{eqnarray} \label{regret-bound4}
	\textrm{Regret}_T \leq \sum_{i=1}^m \sum_{t=1}^T \frac{1}{R_i(t)}\bigg(\sum_{\tau \leq t} \langle x_i(\tau), y_\tau^*-y_\tau \rangle \bigg).
\end{eqnarray}
Note that since the offline policy $\pi^*$ always scores a cache hit for all users, the inner-product is always non-negative, no matter what action sequence $\{y_\tau\}_{\tau \geq 1}$ the online policy takes. Since the cumulative hits $R_i(t)$ is a monotone non-decreasing function for all users under the action of any caching policy, we have $R_i(\tau) \leq R_i(t), \forall \tau \leq t.$ Hence, we can further upper bound the regret from \eqref{regret-bound4} as: 
\begin{eqnarray} \label{reg-bd5}
	\textrm{Regret}_T \leq \sum_{t=1}^T \underbrace{\bigg(\sum_{\tau=1}^t\langle \sum_{i=1}^m \frac{x_i(\tau)}{R_i(\tau)}, y^*_\tau - y_\tau \rangle \bigg)}_{\textrm{OLO}}. 
\end{eqnarray}  
The term within the braces is the dynamic regret of the online policy corresponding to the offline action sequence $\pi^* \equiv \{y^*_\tau\}_{\tau \geq 1}.$ Now as shown in \ref{hit-rate-lb}, the OEGD policy automatically ensures that $R_i(t) = \Omega(\frac{t}{\log t}).$ Hence, the gradient variation for the OLO problem shown in \eqref{reg-bd5} can be bounded as 
\begin{eqnarray*}
	V_t = \sum_{\tau=2}^t || \sum_{i} \frac{x_i(\tau-1)}{R_i(\tau-1)} - \sum_{i} \frac{x_i(\tau)}{R_i(\tau)} ||_2^2 = O(\sum_{\tau} \frac{\log^2 \tau}{\tau^2}) = O(1),
\end{eqnarray*}
where the last equality follows from the fact that $\int_{1}^\infty \frac{\log^2 x}{x^2} dx =2 < \infty.$
Hence, the OEGD policy \citep[Theorem 1]{zhao2020dynamic} achieves a dynamic regret bound of $O(\sqrt{1+ P_t})$.  Hence, assuming 
\[ \sum_{t=1}^T \sqrt{1+P_t} = o(T \log T), \]
the proposed policy asymptotically achieves the optimal objective value. 
\fi
\iffalse
\section{Static Regret of the Online Policy }
We now return to the case of static regret where the offline caching configuration $y^*$ remains fixed in time. Now, for each $i, t,$ we define two exhaustive and mutually exclusive  events: 
\begin{eqnarray*}
	G_{i,t} = \langle x_i(\tau), y^*-y_\tau \rangle < 0, \\
	B_{i,t} = \langle x_i(\tau), y^*-y_\tau \rangle \geq 0.
\end{eqnarray*}
Intuitively, on occurence of the event $G_{i,t},$ the online policy does strictly better than the offline static benchmark in terms of scoring cache hits for the $i$\textsuperscript{th} user on round $t$. On the other hand on occurrence of the event $B_{i,t}$ the benchmark does at least as good as the online policy in terms of scoring a cache hit on the $i$\textsuperscript{th} user. Then we can express the above regret upper bound as:
\begin{eqnarray*}
	\textrm{Regret}_T &\leq& \sum_{t=1}^T \sum_{i=1}^m \frac{1}{R_i(t)} \bigg(\sum_{\tau \leq t} \langle x_i(\tau), y^*-y_\tau \rangle \bigg) (\mathds{1}(B_{i,\tau}) + \mathds{1}(G_{i,\tau})) \\
	& \leq & \sum_{t=1}^T \bigg( \sum_{\tau \leq t} \langle \sum_{i=1}^m \frac{x_i(\tau)}{R_i(\tau)}, y^*-y_\tau \rangle \mathds{1}(B_{i,\tau}) \bigg)
\end{eqnarray*}

\fi
Having established that the $c$-regret of the original problem is upper bounded by the regret of the surrogate learning problem, we now proceed to upper bound the regret of the surrogate problem under the action of a \emph{no-regret} learner. In the sequel, we use the projected Online Gradient Ascent (OGA) policy with adaptive step sizes \citep[Algorithm 2.2]{orabona2019modern}. We call the resulting caching policy \textsc{Online Proportional Fair Caching} (\texttt{OPFC}) policy. The term \emph{Proportional Fair} signifies the fact that the request of the $i$\textsuperscript{th} user is weighted down by a factor of $R_i^\alpha(t)$. In designing the \texttt{OPFC} policy, we have used the fact that the Euclidean diameter of the feasible set $\Delta^N_k$ is bounded by $\sqrt{2k}$ (shown in Lemma \ref{dia-bound}). The pseudocode for this policy is shown in Algorithm \ref{OPFC}. 
\paragraph{Technical insight:}
Note that a tight regret analysis of the \texttt{OPFC} policy is highly non-trivial as the norms of the future gradients are implicitly controlled by the past caching actions. This is different from the standard OCO problems where the upper bound on the norm of the gradients is fixed a priori for all policies. Hence, a tight regret analysis should exploit the fact that, under the \texttt{OPFC} policy, the norm of the gradients diminishes at an appropriate rate. Theorem \ref{reg-bd-alpha} gives a tight regret bound for the surrogate problem. The proof makes use of a new \emph{Bootstrapping} technique for a tight regret analysis.
% We now prove the following regret bound for the surrogate problem. 
%\section{Regret analysis of the Surrogate Problem} \label{hit-rate-lb}
\begin{framed}
\begin{theorem} \label{reg-bd-alpha}
	The \texttt{OPFC} policy described in Algorithm \ref{OPFC} achieves the following static regret bound for the surrogate problem \eqref{surr-regret} for the $\alpha$-fair utility function:
	\begin{eqnarray*}
	\hat{\textrm{Regret}}_T  = \begin{cases}
	O(T^{1/2-\alpha}) ~~ \textrm{if} ~~0<\alpha <\nicefrac{1}{2}, \\
		O(\sqrt{\log T})~~ \textrm{if} ~~\alpha=\nicefrac{1}{2}\\
		O(1) ~~ \textrm{if} ~~\nicefrac{1}{2}<\alpha <1,
	\end{cases}
\end{eqnarray*}
	
	 Furthermore, under this policy, the cumulative hit rates of each user increases linearly with time, \emph{i.e.,} $R_i(T)=\Omega(T), \forall i, T$.  
	%and ensures that $R_i(t) \geq \Omega(\frac{t}{\log t}), \forall i, t.$
\end{theorem}
\end{framed}
\begin{proof}
%In this section, we establish that the OGD policy achieves $O(1)$ regret for $\alpha$-fair utility functions.
%for the logarithmic utility function and simultaneously achieves almost linearly many hit rates for all users. 
%the causal online caching policy that solves a causal version of the OLO problem \eqref{olo-red} with $w_i(\tau) \gets \frac{1}{R_i(\tau)}, \forall i$ scores almost linearly many cache hits with respect to time for each user. 
%The causal OCO policy with the above rate can also be seen to be an instance of a \emph{Proportional Fair} policy, that prioritizes the users in inverse proportion to their current hit rates. 
Using the data-dependent static regret bound achieved by the OGD policy with adaptive step sizes \citep[Theorem 4.14]{orabona2019modern}, the regret for the surrogate problem for the $\alpha$-fair utility function can be upper bounded as follows:
%\begin{eqnarray*}
%	\reg = O\bigg(\sqrt{\sum_{t=1}^T ||\bm{g}_t||_2^2}\bigg)
%\end{eqnarray*}
%where $||\bm{g}_t||_2$ denotes the $\ell_2$ norm of the reward function at round $t$. In our case, the above theorem yields 
%
\begin{eqnarray} \label{adaregret}
	\hat{\textrm{Regret}}_T = O\bigg(\sqrt{\sum_{t=1}^T\sum_i \phi'(R_i(t))^2}\bigg) = O\bigg(\sqrt{\sum_{t=1}^T\sum_i \frac{1}{R_i(t)^{2\alpha}}}\bigg).
\end{eqnarray}
Clearly, the regret bound depends on the dynamics of the cumulative hit rates $\{\bm{R}(t)\}_{t \geq 1}$, which itself is implicitly controlled by the online learner. By the definition of regret, 
%By virtue of the sublinear regret property of the OGD policy, 
for any fixed caching configuration $y^* \in \Delta^N_k,$ we have for any time step $T$: 
\begin{eqnarray} \label{reg-ineq}
	\sum_{t=1}^T \sum_{i} \langle \phi'(R_i(t)) x_i(t), y_t \rangle  \geq \sum_{t=1}^T \sum_i \langle \phi'(R_i(t)) x_i(t), y^* \rangle - \hat{\textrm{Regret}}_T, 
\end{eqnarray} 
where $\hat{\textrm{Regret}}_T$ denotes the worst-case cumulative regret of the adaptive OGD policy up to time $T$. Since the cumulative hits of each user is monotonically non-decreasing, we have:
\begin{eqnarray} \label{bd0}
	R_i(T) \geq 1, \forall i, \forall T.
\end{eqnarray}
This can be ensured by properly initializing the system such that, at round $0,$ all users request the same file (say file $1$) and the policy caches that file.  
Substituting this bound to the regret bound in \eqref{adaregret}, we obtain our first (loose) upper-bound for the regret of the fair caching problem \eqref{surr-regret}:
\begin{eqnarray} \label{reg-bd1}
	\hat{\textrm{Regret}}_T = O(\sqrt{T}).
\end{eqnarray}
Note that this bound might be vacuous as the objective function itself could be smaller in magnitude than this regret bound. A closer inspection reveals the source of this looseness - the cumulative hit lower bound \eqref{bd0} is too loose for our purpose. 

We now strengthen the above upper-bound using a novel \emph{bootstrapping} method, that \emph{simultaneously} tightens the lower bound for the cumulative hits \eqref{bd0} and, consequently, improves the regret upper bound \eqref{adaregret}. 
%\newpage
\iffalse
\hrule
\textbf{Note} The actual regret bound could be better than $O(\sqrt{T}).$ Because if the $R_i(T)'s$ increase linearly, then the magnitude of the gradients increase linearly as well. Upon using the regret bound in terms of the gradients, this yields an $O(1/\sqrt{T})$ regret bound for large $T$. 
\hrule
 \fi
 
 Using the fact that $\langle x_i(t), y_t \rangle = R_i(t+1)-R_i(t),$ and following the same steps as \eqref{bd2}, we have
 \begin{eqnarray}\label{hit-bd1}
 	\sum_{i} \sum_{t=1}^T \phi'(R_i(t)) \langle  x_i(t), y_t \rangle  \leq \sum_i \phi(R_i(T)). 
 \end{eqnarray}
 Furthermore, lower bounding $\phi'(R_i(t))$ by $\phi'(R_i(T)),$ we have
 \begin{eqnarray} \label{hit-bd2}
 	\sum_{t=1}^T \sum_i \langle \phi'(R_i(t)) x_i(t), y^* \rangle \geq \sum_i \phi'(R_i(T)) R_i^*(T),
 \end{eqnarray}
 where $R_i^*(T)\equiv \sum_{t=1}^T \langle x_i(t), y^*\rangle$ is the cumulative hit accrued by a fixed caching configuration $y^* \in \Delta^N_k$ up to time $T.$  Choosing $y^*=\frac{k}{N} \mathds{1}_N,$ we have $R_i^*(T) \geq \frac{kT}{N}, \forall i.$ Hence, combining \eqref{hit-bd1}, \eqref{hit-bd2}, and \eqref{reg-ineq}, we have 
 \begin{eqnarray} \label{oco-prop}
 	\sum_i \phi(R_i(T)) \geq \frac{kT}{N}\sum_i \phi'(R_i(T)) - \hat{\textrm{Regret}}_T.
 \end{eqnarray}
 %inequality \eqref{reg-ineq} yields: 
%\begin{eqnarray} \label{oco-prop}
%	\sum_i \log R_i(T) = \sum_i \int_{1}^{R_i(T)} \frac{dR_i(t)}{R_i(t)} 
%	\geq  \sum_i \sum_{t=1}^T \frac{R_i(t+1)-R_i(t)}{R_i(t)} \geq   \sum_i \frac{\textsf{OPT}_i(T)}{R_i(T)} - \reg, 
%\end{eqnarray}
%where we have used the fact that the cumulative hits $R_i(t)$'s are monotone non-decreasing and $\textsf{OPT}_i(T)$ denotes the cumulative hits of the $i$\textsuperscript{th} user obtained by any fixed offline policy $y^*.$ Recall that inequality \eqref{oco-prop} is valid for any fixed caching configuration $y^* \in \Delta^N_k$. Hence, taking uniform average over all fixed cache configurations obtained by randomly selecting each item with uniform probability, we have that \[\textsf{OPT}_i(T) \geq \beta T, \forall i\] for $\beta \equiv \frac{k}{N}>0.$  Hence, the OEGD policy yields the following performance bound:
%\begin{eqnarray} \label{func-ineq1}
%	\frac{1}{T} \sum_i \log R_i(T) \geq \beta \sum_i \frac{1}{R_i(T)} - \frac{\reg}{T}.
%\end{eqnarray}
Since $0<R_i(T) \leq T, \forall i,$ and $\phi(\cdot)$ is monotone non-decreasing, for any user $i \in [m]$, the above inequality yields:
\begin{eqnarray*}
	\frac{m}{(1-\alpha)T^\alpha} \geq \frac{k}{NR_i^\alpha(T)} - \frac{\hat{\textrm{Regret}}_T}{T}. 
\end{eqnarray*}
\emph{i.e.},
%\begin{eqnarray*}
%	\frac{\reg + m \log T}{T} \geq \frac{k}{N} \frac{1}{R_i(T)}.
%\end{eqnarray*} 
\begin{eqnarray} \label{R-lb}
	R_i^\alpha(T) \geq \frac{k}{N}\bigg(\frac{\hat{\textrm{Regret}}_T}{T} + \frac{m}{1-\alpha}T^{-\alpha}\bigg)^{-1} = \Omega(T^{\min(1/2, \alpha)}), \forall i\in [m],
\end{eqnarray}
where we have used our previous upper bound \eqref{reg-bd1} on the regret. Eqn.\ \eqref{R-lb} is our key equation for carrying out the bootstrapping process as it lower bounds the minimum cumulative hits of users in terms of the worst-case regret. Now we consider two cases:
%, we have, $\reg = O(\sqrt{T}),$ the previous estimate yields:

\begin{figure}
\centering
	\includegraphics[scale=0.45]{technique.pdf}
\put(-70,70){Improve the}
\put(-75,58){lower bound to}
\put(-59, 46){hits $\bm{R}(t)$}
\put(-222,70){Improve the}
\put(-228, 58){upper bound to}
\put(-214, 46){$\hat{\textrm{Regret}_t}$}
\caption{Illustrating the new \emph{Bootstrapping} technique used in the proof of Theorem \ref{reg-bd-alpha}}
\end{figure}

\textbf{Case-I: $0\leq \alpha \leq \nicefrac{1}{2}$}

In this case, we immediately have $R_i(T)=\Omega(T), \forall i,T.$ Substituting this bound on \eqref{adaregret}, we have 
\begin{eqnarray*}
	\hat{\textrm{Regret}}_T  = \begin{cases}
		O(\sqrt{\log T})~~ \textrm{if} ~~\alpha=1/2\\
		O(T^{1/2-\alpha}) ~~ \textrm{if} ~~0<\alpha <1/2.
	\end{cases}
\end{eqnarray*}
\textbf{Case-II: $\nicefrac{1}{2} < \alpha <1$}

In this case, using the bound \eqref{R-lb}, we have $R_i(T)=\Omega(T^{1/2\alpha}), \forall i,T.$ Using the regret bound \eqref{adaregret}, the regret can be bounded as
\begin{eqnarray*}
	\hat{\textrm{Regret}}_T = O(\sqrt{\sum_{t=1}^T \frac{1}{t}})= O(\sqrt{\log T}).
\end{eqnarray*}
Substituting this bound again in \eqref{R-lb}, we have $R_i(T) \geq \Omega(T).$ This, in turn, yields the following regret bound:
\begin{eqnarray*}
	\hat{\textrm{Regret}}_T = O\big(\sqrt{\sum_{t=1}^T \frac{1}{t^{2\alpha}}}\big)=O(1).
\end{eqnarray*}


%\begin{eqnarray} \label{bd1}
%	R_i(T) = \Omega(\sqrt{T}).
%\end{eqnarray}
%%This implies that the difference between two successive gradients is 
%%\begin{eqnarray*}
%%	 ||\sum_i \frac{x_i(t)}{R_i(t)} - \sum_i \frac{x_i(t-1)}{R_i(t-1)}||_2 \stackrel{\textrm{(Triangle ineq.)}}{\leq} \sum_i O(\frac{1}{\sqrt{t}})= O(\frac{1}{t^{1/2}}).
%%\end{eqnarray*}
%Upon combining \eqref{adaregret} with the new lower bound \eqref{bd1} for the cumulative hits, and using Theorem \ref{adaptive-regret}, we can now boost the previous regret bound \eqref{reg-bd1} to arrive at the following tighter bound: 
%\begin{eqnarray} \label{reg-bd2}
%	\reg = O\bigg(\sqrt{\sum_{t=1}^T} \frac{1}{t}\bigg)= O(\sqrt{\log T}).
%\end{eqnarray}
%Substituting the new regret bound in \eqref{func-ineq1}, we arrive at the following lower bound for cumulative hits:
%\begin{eqnarray*}
%	R_i(T) = \Omega\big(\frac{T}{\log T}\big), \forall i. 
%\end{eqnarray*} 
%Using the regret bound \eqref{adaregret} one more time, we have the following final upper bound on regret
%\begin{eqnarray*}
%	\textrm{Reg}(T) = O(\sqrt{\sum_{t=1}^T \frac{(\log t)^2}{t^2}})=O(1). 
%\end{eqnarray*}
\end{proof}
Finally, combining Theorem \ref{regret-comp} and Theorem \ref{reg-bd-alpha} together, yields a sublinear $1.445$-regret bound for the \textsf{OFC} problem. 

 
\textbf{Note:} 

1. Observe that the regret bound given by Theorem \ref{reg-bd-alpha} always remains non-vacuous, \emph{irrespective} of the value of the parameter $\alpha$ and the file requests. This is because, irrespective of the file request sequence, by choosing the constant action $y=\nicefrac{k}{N}\mathds{1}_N,$ each user can achieve a hit rate of $\frac{k}{N}T.$ Hence, the optimal offline value of the $\alpha$-fair utility function $\Omega(T^{1-\alpha}).$ On the other hand, the \texttt{OPFC} policy achieves a regret bound that is always dominated by the optimal static offline objective.


2. It is not surprising that the policy \texttt{OPFC} achieves a constant regret in the regime $1/2 < \alpha <1.$ It can be easily verified that, for $\alpha=1$ (which corresponds to the logarithmic utility function), the oblivious randomized policy, which caches $k$ files chosen uniformly at random out of $N$ files at each round, achieves constant regret. 

3. In the special case of $\alpha=0,$ the \texttt{OFC} problem corresponds to the cumulative hit rate maximization problem for all users. Hence, Theorem \ref{reg-bd-alpha} recovers the well-known $O(\sqrt{T})$ regret bound for online caching established in \cite{SIGMETRICS20}.


\subsubsection{In-expectation regret bound for the \texttt{OPFC} policy with integral caching}
Theorem \ref{reg-bd-alpha} establishes $c$-Regret guarantee for the \texttt{OPFC} policy when the caching variables are allowed to be fractional. We now establish the same regret guarantee in expectation when the policy is allowed to cache whole files only. In this case, given the fractional caching vector $y_t \in \Delta^N_k$ on round $t$, the \texttt{OPFC} policy uses Madow's sampling (given in Algorithm \ref{Madow}) to randomly sample a subset $Y_t \in \{0,1\}^N$ consisting of $k$ distinct files according to the inclusion probability vector $y_t.$ 

Let $\{\mathcal{F}_t\}_{t \geq 1}$ be the natural filtration given by $\mathcal{F}_t= \sigma(Y_1, Y_2, \ldots, Y_t), t\geq 1.$ 
%We now claim that, under the action of the \texttt{OPFC} policy, the quantity $\mathbb{E} \big[\phi'(\mathsf{R}_i(t))\big]$ in the above equation can be replaced by $\phi'(R_i(t))$ without blowing up the regret bound too much. 
Taking expectation of both sides of Eqn.\ \eqref{regret-comp-eq}, we have 
\begin{eqnarray*} \label{discrete-1}
	\mathbb{E}(c-\textrm{Regret}_T) &\leq& \mathbb{E} \sum_{t=1}^T \bigg( \sum_{i}\langle \phi'(\mathsf{R}_i(t)) x_i(t), y^*- Y_t \rangle \bigg)\\
	&\stackrel{(a)}{=}& \sum_{t=1}^T \sum_{i} \bigg(\mathbb{E} \langle \phi'(\mathsf{R}_i(t)) x_i(t), y^*\rangle - \mathbb{E} \langle \phi'(\mathsf{R}_i(t)) x_i(t), Y_t\rangle \bigg) \\
	&\stackrel{(b)}{=}& \sum_{t=1}^T \sum_{i}\bigg( \langle \mathbb{E}\phi'(\mathsf{R}_i(t)) x_i(t), y^*\rangle - \mathbb{E} \mathbb{E} \langle \phi'(\mathsf{R}_i(t)) x_i(t), Y_t|\mathcal{F}_t\rangle \bigg) \\
	&\stackrel{(c)}{=}& \sum_{t=1}^T\sum_{i}\bigg( \langle \mathbb{E}\phi'(\mathsf{R}_i(t)) x_i(t), y^*\rangle - \mathbb{E}  \langle \phi'(\mathsf{R}_i(t)) x_i(t), \mathbb{E}(Y_t|\mathcal{F}_t)\rangle \bigg)\\
	&\stackrel{(d)}{=}& \sum_{t=1}^T\sum_{i}\bigg( \langle \mathbb{E}\phi'(\mathsf{R}_i(t)) x_i(t), y^*\rangle - \langle \mathbb{E}\phi'(\mathsf{R}_i(t)) x_i(t), y_t\rangle \bigg) \\
	&\stackrel{(e)}{\leq}& \sum_{t=1}^T \sum_{i}\bigg( \langle \mathbb{E}\phi'(\mathsf{R}_i(t)) x_i(t), y^*\rangle - \langle \phi'(R_i(t)) x_i(t), y_t\rangle \bigg).
\end{eqnarray*}
where in (a), we have used the linearity of expectation, in (b), we have used the tower property of expectation, in (c), we have used the fact that each of the $\mathsf{R}_i(t)$ random variables is $\mathcal{F}_t$ measurable, in (d), we have used the fact that Madow's sampling procedure gives an exact sample with inclusion probability vector $y_t$, \emph{i.e.,} $\mathbb{E}(Y_t|\mathcal{F}_t)=y_t,$ and, finally in (e), we have used Jensen's inequality using the convexity of the function $\phi'$ and the fact that $\mathbb{E}(\mathsf{R}_i(t)) = R_i(t).$
%random variable that evolves according to Eqn.\ \eqref{reward-evolution} where the continuous variables $y_t$'s are replaced by their random realizations $Y_t.$ Using the linearity and tower property of expectation, the above inequality yields
%\begin{eqnarray*}
%	\mathbb{E}(c-\textrm{Regret}_T) &\leq& \sum_{t=1}^T \bigg(  \sum_{i}\mathbb{E} \big[ \mathbb{E}\langle\phi'(\mathsf{R}_i(t)) x_i(t), y^*- Y_t \rangle |\mathcal{F}_t) \big]\bigg)\\
%	&\stackrel{(a)}{=}&\sum_i \sum_{t=1}^T \bigg( \langle \mathbb{E} \big[\phi'(\mathsf{R}_i(t))\big] x_i(t), y^*- y_t \rangle \bigg),
%\end{eqnarray*}
%where, in (a), we have used the facts that the r.v. $\mathsf{R}_i(t)$ is $\mathcal{F}_t$ measurable
% and $\mathbb{E}(Y_t|\mathcal{F}_t) = y_t$. Due to the linearity of the state evolution \eqref{reward-evolution}, we have that $\mathbb{E}(\mathsf{R}_i(t)) = R_i(t), \forall i,t.$ 

\begin{lemma}[Concentration bound]
\begin{eqnarray*}
		|\mathbb{E}\phi'(\mathsf{R}_i(t)) - \phi'(R_i(t))| \leq  
\end{eqnarray*}
\end{lemma}

\begin{proof}
	Note that the random variables $\{Y_t\}_{t \geq 1}$ are \emph{not} independent. This is because, the the action of the \texttt{OPFC} policy $Y_t$ on round $t$ depends on its actions on the previous rounds (through the cumulative hit variable). However, from Eqn.\ \eqref{reward-evolution}, it is clear that when any one of the first $t$ r.v.s change, the value cumulative hit $R_i(t)$ may change by at most $1$. Hence, using McDiarmid's bounded distance inequality \citep{boucheron2013concentration}, we conclude that 
	\begin{eqnarray*}
		\mathbb{P}(|\mathsf{R}_i(t) - R_i(t)| \geq \lambda ) \leq \exp(-2\lambda^2/t), 
	\end{eqnarray*} 
	where we have used the fact that $\mathbb{E}(\mathsf{R}_i(t))= R_i(t).$ Now, fix some $\lambda = t^{3/4}$ and recall from Theorem \ref{reg-bd-alpha} that, under the action of \texttt{OPFC} policy, $R_i(t)= \Omega(t).$ Using these, we have 
	\begin{eqnarray*}
		|\mathbb{E}\phi'(\mathsf{R}_i(t)) - \phi'(R_i(t))|&=&|\mathbb{E} \frac{1}{\mathsf{R}_i^\alpha(t)}- \frac{1}{R_i^\alpha(t)}| \\
		&\stackrel{(a)}{\leq} & \frac{1}{(R_i(t) - \lambda)^\alpha}-\frac{1}{R_i(t)^\alpha} + \exp(-2\lambda^2/t) \\
		&\leq & \frac{R_i(t)^\alpha - (R_i(t)-\lambda)^\alpha}{R_i^{2\alpha}(t)} + \exp(-2\lambda^2/t) \\
		&\stackrel{(b)}{\leq} & \frac{\lambda^\alpha}{R_i^{2\alpha}(t)} + \exp(-2\lambda^2/t)
	\end{eqnarray*}
	where, in (a), we have used the fact that $R_i(t)\geq 1, \forall t$, and in (b), we have made use of the inequality $(a+b)^\alpha \leq a^\alpha + b^\alpha, \forall 0\leq \alpha \leq 1.$
	
	
\end{proof}


\iffalse
\section{An Alternative Reward Structure}
We consider the reward only at the end of the horizon, \emph{i.e.,} the regret of a policy is defined as
\begin{eqnarray*}
	\textrm{Reg}(T) \equiv \sum_i \phi (R_i^*(T)) - \sum_i \phi (R_i(T)),
\end{eqnarray*}
where $\phi$ is some non-decreasing concave function. Note that, we recover the cumulative hit rate maximization problem by taking the utility function $\phi$ to be $\phi(x)=x.$ We want to design a policy with a non-trivial regret bound. 

\fi

%Note that the weight $w_i(\tau)$ can be alternatively expressed as $w_i(\tau) = \sum_{t=1}^T \frac{1}{R_i(t)} - \sum_{t=1}^{\tau-1} \frac{1}{R_i(t).}$ In this expression, the first term is unknown but the second term is known at time $\tau.$ We can either use the principle of optimism in the face of uncertainty or doubling trick to estimate the quantities $w_i(\tau)$ and run an OLO policy to guarantee an $O(\sqrt{T})$-regret. 


%\subsection{A Naive Policy}
%Since the cumulative hits of each user are non-decreasing with time, we have the following crude estimate $w_i(\tau) \leq \frac{T-\tau+1}{R_i(\tau)-1}, \forall i.$ Hence, the problem \eqref{olo-red} corresponds to an online linear optimization problem where the reward vector at step $\tau$ is given by 
%\begin{eqnarray*}
%	\bm{g}_\tau = (T-\tau+1)\sum_{i} \frac{\bm{x}_i(\tau)}{R_i(\tau)-1}. 
%\end{eqnarray*}
%In principle, it is possible to design an online caching policy using the framework designed in \cite{mukhopadhyay2022k}. 
%However, since the gradients can not be bounded reasonably, the usual analysis fails to yield a sublinear regret bound. 

%\subsection{A No-regret fair caching policy}
%Let's now make the assumption that the hit rates of the users converge under the action of the given policy. In other words, 
%Clearly, the weight vector $\bm{w}(\tau)$ at time $\tau$ depends on the future file request sequence from the users, and, as such, the problem \eqref{regret-def} is \emph{not} an instance of the standard OCO problem. On the other hand, we make the critical observation that if the weights can be appropriately controlled under the action of a given online policy, the problem \eqref{regret-def} can be reduced to a standard OCO problem. In the following, we consider a causal OCO policy that simply ignores all future terms in the weight function. 
%Towards this, we confine our attention to the class of online caching policies $\Pi_{\bm{\alpha}}$ where
%\begin{eqnarray} \label{rate-constraint}
%	w_i(\tau) = O(\ln (T)). 
%\end{eqnarray} 
%there exist strictly positive numbers $\{\alpha_i\}_{i=1}^m$ with $0<\alpha_i\leq 1, \forall i,$ s.t. w.h.p. 
%\begin{eqnarray} \label{rate-constraint}
%	 \frac{R_i(t)}{t} \geq  \alpha_i, ~~ \forall i,t . 
%\end{eqnarray} 
%where the expectation is taken with respect to the randomness of the policy. 
\iffalse
\subsection{A class of policies guaranteeing constraint \eqref{rate-constraint}}
%Note that \eqref{rate-constraint} is not a very restrictive assumption as an 
Consider a randomized caching policy $\pi$ that, at every round, caches $C$ files uniformly at random with probability $\epsilon,$ and runs some other online caching policy $\pi^{\textrm{OCO}}$ (to be described later) with probability $1-\epsilon.$ Since the cumulative hits $R_i(t)$'s are non-decreasing with time, the following theorem shows that the policy $\pi$ satisfies the constraint \eqref{rate-constraint} with some admissible $\bm{\alpha},$ irrespective of the policy $\pi^{\textrm{OCO}}.$ The proof is deferred to the Appendix.

%\begin{appendixproof}
%Proof of the theorem.	
%\end{appendixproof}
%
%\begin{theoremrep}
\begin{theorem}
The randomized policy $\pi$ guarantees constraint \eqref{rate-constraint} w.h.p. 
%\end{theoremrep}
\end{theorem}
For any fixed $0\leq \delta <1$ and starting from any round $\tau,$
divide the remaining rounds into successive \emph{frames} where each frame consists of consecutive $\lambda$ rounds. We make the following claim:
\begin{proposition} \label{hit-prop}
	Upon setting the frame length $\lambda \equiv \frac{1}{\epsilon C/N}\ln (m/\delta),$ in any future frame, all users receive at least one cache hit with probability at least $1-\delta.$
\end{proposition}

\begin{proof}
Note that \emph{irrespective} of the particular file requested (which could be adversarial), due to the randomized exploration, on every round, each user receives a cache hit with probability at least $\epsilon C/N.$
	 Now, for any user $i$, let $\mathcal{E}_{i}$ be the event denoting that the $i$\textsuperscript{th} user receives at least one hit in any given future frame. Then we have:
	\begin{eqnarray*}
		\mathbb{P}(\mathcal{E}_{i}^c) \leq \bigg(1- \epsilon \frac{C}{N}\bigg)^\lambda \leq e^{-\epsilon \lambda C/N}.  
	\end{eqnarray*}
Hence,
	\begin{eqnarray*}
		\mathbb{P}(\cap_{i=1}^m \mathcal{E}_{i})=1- \mathbb{P}(\cup_{i=1}^m \mathcal{E}^c_{i}) \stackrel{(a)}{\geq} 1-me^{-\epsilon \lambda  C/N} \stackrel{(b)}{\geq} 1-\delta,
	\end{eqnarray*}
	where in (a) we have used the union bound and (b) follows upon setting $\lambda = \frac{1}{\epsilon C/N}\ln (m/\delta).$ 
	\end{proof}
	
	%The above implies that \emph{all} users receive at least one cache hit in every frame with probability at least $1-\delta.$ 
	Let $\{\mathcal{F}_j\}_{j=1}^T$ be the natural filtration generated by the policy. We now make the following claim:
	\begin{proposition} \label{hp-bound}
	On any round $\tau,$ we have
	  \[\mathbb{P}\bigg[\frac{1}{R_i(\tau)} \leq w_i(\tau) \leq \frac{\lambda}{R_i(\tau)} + \ln\big(1+T\big), \forall i \bigg|\mathcal{F}_{\tau-1}\bigg] \geq 1-\frac{\delta T}{\lambda},\] where the parameter $\lambda$ was chosen as in Proposition \ref{hit-prop}.
	\end{proposition}
	\begin{proof}
	Recall that 
	\begin{eqnarray*} 
			 w_i(\tau) = \sum_{t=\tau}^T \frac{1}{R_i(t)},
	\end{eqnarray*}
	from which the first bound follows immediately. 
 Let $t_j$ denote the index of the first round of the subsequent $j$\textsuperscript{th} frame with $t_1=\tau$. Since the variables $\{R_i(t)\}_t$ are non-decreasing, we can upper-bound $w_i(\tau)$ as 
	\begin{eqnarray} \label{weight-def}
		w_i(\tau) \leq \lambda \sum_{j=1}^{\frac{T-\tau}{\lambda}} \frac{1}{R_i(t_j)}.
	\end{eqnarray}
	From Proposition \ref{hit-prop} and using a union bound over all subsequent frames, we have with probability at least $1- \delta (T-\tau)/\lambda \geq 1-\frac{\delta T}{\lambda}:$
	\begin{eqnarray*}
		R_i(t_j) \geq R_i(\tau) + j-1, ~~ \forall i,j.
	\end{eqnarray*}
	Hence, with probability at least $1-\nicefrac{\delta T}{\lambda}$ conditioned on the past, the weight \eqref{weight-def} can be upper bounded as 
	\begin{eqnarray*}
		w_i(\tau)&\leq& \lambda \sum_{j=1}^{\frac{T-\tau}{\lambda}} \frac{1}{R_i(\tau)+j-1} \\
		&\leq& \frac{\lambda}{R_i(\tau)} + \lambda  \int_{0}^{\frac{T-\tau}{\lambda}} \frac{dx}{R_i(\tau)+ x} \\
		&=& \frac{\lambda}{R_i(\tau)}+ \lambda \ln \bigg(1+ \frac{T-\tau}{\lambda R_i(\tau)}\bigg)\\
		&\leq& \frac{\lambda}{R_i(\tau)}+ \lambda \ln T~~ \forall i.
	\end{eqnarray*}
	where the last inequality follows from the fact that $\lambda \geq 1, R_i(\tau) \geq 1, \forall i, \tau \geq 1,$ and the monotonicity of the cumulative hits.
	\end{proof}
	
	%The above result readily yields an upper bound on the conditional expectation of the weight vector at time $\tau.$
Using a union bound once again, Proposition \ref{hp-bound} implies that with probability at least $1-\frac{\delta T^2}{\lambda},$ the regret bound \eqref{olo-red} can be further upper-bounded as:
\begin{eqnarray*}
	\mathcal{R}_T \leq \sum_{\tau=1}^T \langle \sum_{i} x_i(\tau) w_i(\tau), y^*- y_\tau \rangle,
\end{eqnarray*}

%as shown below. 
%, the condition \eqref{rate-constraint} can be ensured if at each round, with a small probability $\epsilon,$ we play the policy $\pi^{\textsc{RAND}},$ and with the complementary probability, we play any other online caching policy. 

%For large $\tau,$ a rough estimate for $\alpha_i$ is given by $\frac{R_i(\tau)}{\tau}.$ (To get rid of the expectations, the exploration can also be done on deterministic rounds. The regret bound should not change by more than a constant factor.)
%With this assumption, we have the following upper bound for the weight function
%\begin{eqnarray*}
%	w_i(\tau) \leq \frac{\tau}{R_i(\tau)} \sum_{t=\tau}^T \frac{1}{t} \leq \frac{\tau \ln (T/\tau)}{R_i(\tau)} \leq \frac{\ln(T)}{R_i(\tau)/\tau}.
%\end{eqnarray*}
%This yields $w_i(\tau)= O(\frac{\ln T}{\alpha_i}).$ 
Hence, the online fair caching problem reduces to an OLO problem with the following reward vector at time $\tau:$ 
\begin{eqnarray*}
	\bm{g}_\tau = \ln(T) \sum_i \frac{\bm{x}_i(\tau)}{R_i(\tau)/\tau}.
\end{eqnarray*}
The above is the same as the online caching problem where the cache-hits are discounted by the current hit-rates, inducing fairness among the users. 
Since $|| \bm{g}_\tau||_2 \leq \ln(T)(\sum_{i}\frac{1}{\alpha_i})$, using the online caching policy described in \cite{mukhopadhyay2022k}, we get the following sublinear regret guarantee:
\begin{eqnarray*}
	\mathcal{R}_T \leq 2\frac{\ln T}{\epsilon} (\sum_i \frac{1}{\alpha_i})\sqrt{2CT\ln \frac{N}{C}} + \epsilon m T \ln T,
\end{eqnarray*} 
where the last term is an upper bound on the expected regret incurred due to the uniform exploration. By optimizing over $\epsilon,$ we get a policy with $\tilde{O}(T^{3/4})$ regret. 

\textbf{TODO} 
\begin{enumerate}
	\item It is probably unnecessary to do uniform exploration to ensure the constraint \eqref{rate-constraint}. I think, the policy $\pi^{\textrm{OCO}}$ does sufficient exploration on its own to ensure \eqref{rate-constraint}. If we can get rid of the exploration part, we will have a policy with $O(\sqrt{T})$ regret. 
	\item Also, it would be interesting to carry out the above analysis for $\alpha-$fair utility functions.
	\item After proving the sublinear regret bound, we may iterate the regret bound again to obtain tighter bounds for $\vec{\bm{\alpha}}.$
	\item  Strengthening of Theorem 1 using Doob-Kolmogorov Maximal inequality.
\end{enumerate}


\subsection{Observation-I}
%By switching the order of summations, the regret upper bound \eqref{olo-red} can be alternatively expressed as :
Recall that from Eqn.\ \eqref{first-order-bound}, the regret for any policy can be bounded as:
\begin{eqnarray} \label{regret-expr2}
	\textrm{Regret}_T \leq \sum_{i=1}^m \sum_{t=1}^T \frac{1}{R_i(t)} \bigg(\sum_{\tau \leq t} \langle x_i(\tau), y^*-y_\tau \rangle \bigg).
\end{eqnarray}
The inner summation is simply the regret of a policy up to round $t$ for the linear hit-rate maximization problem $\mathcal{P}'$ for the $i$\textsuperscript{th} user. 

\fi 
%
%Now suppose that we can come up with an adaptive caching policy $\pi$ which ensures sublinear regret for each users, \emph{i.e.,} for all $y^* \in \Delta^N_k,$ for all time $t \geq 1,$ and all users $i,$ we have:  
%\begin{eqnarray} \label{reg-expr1}
%	\sum_{\tau \leq t} \langle x_i(\tau), y^*-y_\tau \rangle = O(\sqrt{t}). 
%\end{eqnarray} 
%\begin{lemma} \label{rate-lb}
% Under the above policy $\pi,$ for all users $i \in [m],$ we have $R_i(t) \geq \frac{k}{N}t - O(\sqrt{t}), \forall t \geq 1. $
%\end{lemma}
%\begin{proof}
%	Since the regret bound \eqref{reg-expr1} is valid for all $y^* \in \Delta^N_k,$ we have 
%	\begin{eqnarray*}
%		R_i(t)= \sum_{\tau \leq t} \langle x_i(\tau), y_\tau \rangle \geq \sum_{\tau \leq t} \langle x_i(\tau), y^* \rangle - O(\sqrt{t}).
%	\end{eqnarray*}
%	Now taking the uniform average of the RHS over all feasible $y^*,$ we have: 
%	\begin{eqnarray*}
%		R_i(t) \geq \frac{k}{N}t - O(\sqrt{t}).
%	\end{eqnarray*}
%\end{proof} 
%Hence, under the action of the policy $\pi,$ the regret for the original problem can be upper-bounded from \eqref{regret-expr2} as follows:
%\begin{eqnarray*}
%		\textrm{Regret}_T \leq \sum_{i=1}^m \sum_{t=1}^T \frac{O(\sqrt{t})}{\nicefrac{kt}{N}- O(\sqrt{t})} \leq \sum_{i=1}^m \sum_{t=1}^T O(\frac{1}{\sqrt{t}}) = O(\sqrt{T}).
%\end{eqnarray*}
%\subsection{Observation-II}
%
%Using Lemma \ref{rate-lb}, the regret of the policy $\pi$ can be upper bounded as 
%\begin{eqnarray*}
%	\textrm{Regret}_T \stackrel{(a)}{\leq} \sum_{i=1}^m \sum_{t=1}^T O(\sqrt{t})\phi_i' \big(\nicefrac{kt}{N}-O(\sqrt{t}) \big) = O\big(\sum_{i} \int_{1}^T \sqrt{t}\phi'_i(t) dt\big) \stackrel{(b)}{=}  o(T), 
%\end{eqnarray*}
%where inequality (a) follows from Assumption (1) and equality (b) follows from Assumption (2). 
%
\iffalse
\subsection{Designing a No-Regret Fair Caching Policy with Perturbed Requests}
%In this Section, let us denote the file requested on round $t$ by the $i$\textsuperscript{th} user by $z_i(t),  i\in [m], t \in [T].$ 
Fix a small perturbation probability $0 < \epsilon <1,$ to be fixed later \footnote{We will see that $\epsilon \to 0$ as $T \to \infty$.}. Let $\{U_i(t)\}_{t=1}^T$ be a sequence of i.i.d. random variables such that each r.v. is distributed uniformly on the library $[N]$\footnote{$U_i(t)$ can also be replaced by its expectation, \emph{i.e.,} the deterministic vector $\nicefrac{k}{N} \mathds{1}_N$.} Next, for each request sequence $\{x_i(t)\}_{t=1}^T,$ we derive a new perturbed sequence $\{\hat{x}_i(t)\}_{t=1}^T$ as follows:
\begin{eqnarray*}
\hat{x}_i(t) =	\begin{cases}
	 x_i(t), ~~\textrm{w.p.}~~ 1-\epsilon\\
	 U_i(t), ~~\textrm{w.p.}~~ \epsilon. 	
	\end{cases}
\end{eqnarray*}
In our proposed policy, the online learner is fed with the perturbed request sequence $\{\hat{x}_i(t)\}_{t \geq 1}.$  In the following, we will see that the perturbation makes the design and analysis of a no-regret fair caching policy significantly easier. Although, our motivation for perturbing the original request sequence is to aid designing a no-regret policy, the perturbation may also be necessary if the request sequence need to protect the privacy of the users. In this case, the parameter $\epsilon$ is determined by the Differential privacy requirements of the users. 

For the perturbed request sequence $\{\hat{x}_i(t)\}_{t \geq 1},$ the probability of any user receiving a cache hit under any caching policy at any given round is at least $\frac{\epsilon k}{N}.$ Hence, w.h.p. it holds that $\hat{R}_i(t) \geq \frac{\epsilon kt}{N},$ where $\hat{\bm{R}}(t)$ denotes the cumulative hits of all users for the perturbed request sequence. Now consider a \emph{strongly adaptive} online caching policy $\pi$ that achieves $O(\sqrt{t})$ regret for all time $t \in [T],$ where the objective is to maximize the cumulative hits of all users. Hence, the regret upper bound \eqref{regret-expr3} with respect to the \emph{perturbed} file requests can be further upper-bounded as 
\begin{eqnarray*}
	\hat{\textrm{Regret}}_T &\leq& \sum_{t=1}^T \phi'(\epsilon kt/N) \bigg(\sum_{\tau \leq t} \langle \sum_{i} \hat{x}_i(\tau), y^* - y_\tau \rangle \bigg) \\
	&\stackrel{(a)}{=}& O\bigg(\sum_{t=1}^T \sqrt{t} \phi'(\epsilon kt/N) \bigg) \\
	&=& O\bigg( \int_{0}^T \sqrt{t} \phi'(\epsilon kt/N) dt\bigg) \\
	&=& O\bigg( \big(\frac{N}{k \epsilon}\big)^{3/2} \int_{0}^{\epsilon kT/N} \sqrt{x} \phi'(x) dx \bigg)\\
	&\stackrel{(b)}{=}& O\bigg( \big(\frac{N}{k\epsilon} \big)^{3/2} J_\phi\big(\frac{\epsilon k T}{N}\big) \bigg), 
\end{eqnarray*} 
where (a) follows from the property of the no-regret caching policy $\pi,$ and the function $J_\phi$ appearing in (b) has been defined in Condition 2 in Definition \ref{admissible}. 
Clearly, since the function $J(\cdot)$ is sublinear in its argument, the regret of the policy $\pi$ with the perturbed request sequence $\{\hat{\bm{x}}(t)\}_{t \geq 1}$ remains sublinear. 

\begin{algorithm}
\caption{\texttt{OFC} Policy}
\label{uncoded_inelastic}
\begin{algorithmic}[1]

\FOR {$t=1$ to $T$}
\STATE Run a strongly adaptive caching policy (\emph{e.g.,} OGD) to decide the caching configuration $y_t$ for round $t$ that yields a sublinear regret for the OLO problem with per round reward function $q_t(y_t) \equiv \langle \sum_{i=1}^m \hat{x}_i(\tau), y_\tau \rangle .$
\STATE Randomly perturb the file request of each user with probability $\epsilon$ as shown below 
\begin{eqnarray*}
\hat{x}_i(t) =	\begin{cases}
	 x_i(t), ~~\textrm{w.p.}~~ 1-\epsilon\\
	 U_i(t), ~~\textrm{w.p.}~~ \epsilon. 	
	\end{cases}
\end{eqnarray*}
  \ENDFOR
\end{algorithmic}
\end{algorithm}


\textbf{Note:} It is interesting to note that the idea of  perturbing the request sequence is akin to the concept of \emph{smoothed analysis}, where an input instance to an algorithm is randomly perturbed to guarantee an efficient run-time \citep{spielman2004smoothed}.   

\subsection{Regret with respect to the un-perturbed requests}
Now we bound the regret of the above online policy with respect to the original un-perturbed file request sequences. Let $\hat{R}_i(t)$ and $R_i(t)$ denote the number of hits received by the $i$\textsuperscript{th} user up to time $t$ for the perturbed and true sequence respectively. We can write 
\begin{eqnarray*}
	R_i(t) = \sum_{\tau=1}^t \langle x_i(\tau), y_\tau \rangle, ~~ 
	\hat{R}_i(t) = \sum_{\tau=1}^t \langle \hat{x}_i(\tau), y_\tau \rangle. 
\end{eqnarray*} 
Hence,
\begin{eqnarray*}
	\hat{R}_i(t) - R_i(t) = \sum_{\tau=1}^t \langle \hat{x}_i(\tau)-x_i(\tau), y_\tau \rangle \leq \sum_{\tau=1}^t \langle \hat{x}_i(\tau), y_\tau \rangle \mathds{1}(\hat{x}_i(\tau)\neq x_i(\tau)),
\end{eqnarray*}
where the last inequality uses the fact that $\langle x_i(\tau), y_\tau \rangle \geq 0, \forall \tau$. Now taking expectation w.r.t. the perturbation, we conclude that \footnote{There should be an expectation over $\hat{R}_i(t),$ but for simplicity, I am just writing it without the expectation. Rigorously speaking, one needs to establish a high probability bound here.}
\begin{eqnarray*}
	\hat{R}_i(t) - R_i(t) \leq \epsilon \hat{R}_i(t),
\end{eqnarray*}  
which implies that $R_i(t) \geq (1-\epsilon) R_i(t).$
Thus the regret for the original requests for logarithmic utility function is bounded by:
\begin{eqnarray} \label{regret-ub}
	\textrm{Regret}_T \leq 2 \log (1+\epsilon)T + \hat{\textrm{Regret}_T} \leq 2 \epsilon T + O\bigg( \big(\frac{N}{k\epsilon} \big)^{3/2} J\big(\frac{\epsilon k T}{N}\big) \bigg).
\end{eqnarray}
Finally, we can minimize the regret upper-bound \eqref{regret-ub} by optimizing over the perturbation probability $\epsilon.$ As an example, for the logarithmic fairness function, the optimal values are given as follows:
\begin{eqnarray*}
	\epsilon^*_{\textrm{logarithmic}} = \Omega(T^{-1/4}), ~~ \textrm{Regret}_T = O(T^{3/4}).
\end{eqnarray*}
The regret for $\alpha$-fair utility can also be optimized using a similar approach.
%In the case of $\alpha$-fair utility functions, the optimal values are given as follows:
%\begin{eqnarray*}
%	\epsilon^*_{\alpha-\textrm{fair}} = \Omega(T^{\frac{1-2\alpha}{2(1+\alpha)}}), ~~ \textrm{Regret}_T = O(T^{\frac{3}{2(1+\alpha)}}).
%\end{eqnarray*}
Strictly speaking, one needs to know the value of the functional $J_\phi(\cdot)$ to tune the optimal value of $\epsilon.$
\fi

\section{Extensions} \label{ext}
The \texttt{OPFC} policy and its regret analysis goes through for any general non-negative request vectors as well. This might be useful for fair cardinality-constrained portfolio optimization problems.  


\section{Open Problems}
\begin{enumerate}
\item Prove expected regret bounds in the discrete caching set up
	\item Proving tight lower bounds on regret for different values of $\alpha$
	\item Using predictions for the next file requests to reduce the regret bound
	\item Designing policies with small dynamic regret
	\item Approach using adversarial RL
	\item Investigating what happens when the users intermittently come and go. If the user $i$ is not present on round $t$, it simply requests the zero vector.
	%\item Bounds on Dynamic Regret
\end{enumerate}

\section{Appendix}
\subsection{Bounding the Diameter of the Feasible set}
\begin{lemma} \label{dia-bound}
	\[\textrm{Diam}(\Delta^{N}_k) \leq \sqrt{2k}.\]
\end{lemma}

\begin{proof}
	Let $x, y \in \Delta^N_k.$ We have 
	\begin{eqnarray*}
		||x-y||_2^2 = \sum_{i=1}^N (x_i-y_i)^2 = \sum_{i=1}^N |x_i-y_i| |x_i-y_i| \stackrel{(a)}{\leq} \sum_{i=1}^N |x_i-y_i|\stackrel{(b)}{\leq} \sum_{i=1}^N |x_i| + \sum_{i=1}^N|y_i| \stackrel{(c)}{=} 2k,
	\end{eqnarray*}
	where, in (a), we have used the fact that $0\leq x_i, y_i \leq 1,$ in (b), we have used triangle inequality, and in (c), we have used the fact that the sum of the components of each feasible vector is $k$.
\end{proof}


\subsection{Sampling Without Replacement According to a Given Inclusion Probability Vector}

\begin{algorithm} 
\caption{\textsc{Madow-Sample} ($p$)}
\label{Madow}
\begin{algorithmic}[1]
\State \algorithmicrequire{ A universe $[N]$ of size $N$, the cardinality of the sampled set $k$, and a  marginal inclusion probability vector $p \in \Delta^N_k.$}
\State \algorithmicensure{ A random $k$-set $S$ with $|S|=k$ such that, $\mathbb{P}(i \in S)=p_{i}, \forall i\in [N]$} 
\State Define $\Pi_0=0$, and $\Pi_i= \Pi_{i-1}+p_{i}, \forall 1\leq i \leq N.$
\State Sample a uniformly distributed random variable $U$ from the interval $[0,1].$
\State $S \gets \emptyset$
\ForEach {$i\gets 0$ to $k-1$}
\State Select the element $j$ if $\Pi_{j-1} \leq U + i < \Pi_j.$ 
%\State $S \gets S \cup \{j\}.$
\EndForEach
\State \Return $S$
\end{algorithmic}
\end{algorithm}

%Interestingly, the policy $\pi$ would also simultaneously yield sublinear regret for the maxmin fairness function.
%\begin{framed}
%\textbf{Question:} Can we use \textsc{Hedge} as a meta-policy to design the policy $\pi$?
%\end{framed}
%
%\subsection{Policy design with Blackwell's approachability}
%We now use Blackwell's approachability \citep{cesa2006prediction} for designing an online learning policy that guarantees the uniform regret bound \eqref{reg-expr1} in the regime $m \leq C$ \footnote{Provide a counter-example showing that achieving sublinear regret is impossible in the regime $m>C.$} 

%Thus the causal OCO policy \eqref{olo-red}, with $w_i(t) \propto \frac{1}{R_i(t)},$ yields $\tilde{O}({\sqrt{T}})$ regret for the fair caching problem. 
%
%A better estimate may be found directly using Eqn.\ \eqref{func-ineq1}. We may write:
%\begin{eqnarray*}
%	\beta \sum_i \frac{1}{R_i(t)} \leq \frac{1}{t}\sum_i \log R_i(t) + O(\frac{1}{\sqrt{t}}) \leq m \frac{\log T}{t} + O(\frac{1}{\sqrt{t}}).
%\end{eqnarray*}
%Summing up both sides over all rounds, we have the bound:
%\begin{eqnarray*}
%	\beta \sum_{t=1}^T \sum_i\frac{1}{R_i(t)} \leq m \log^2(T) + O(\sqrt{T}).
%\end{eqnarray*}
%The last $O(\sqrt{T})$ can be reduced to $O(1/\sqrt{T}).$

%\subsection{An Online Learning Policy that guarantees the uniform regret bound \eqref{reg-expr1}}
%To show that there does exist an (albeit inefficient) online learning policy that guarantees the uniform regret bound \eqref{reg-expr1}, consider an instance of Learning with Experts advice problem as described below. 
%
%We define a collection of $P=m\binom{N}{k}$ experts such that to each user $i \in [m]$ and each subset files $y \in \binom{[N]}{k},$ we associate a corresponding ``Expert" $\mathcal{E}_{i,y}.$ The reward of the expert $(i,y)$ on round $t$ is defined as $r_{i,y} = \langle x_i(t), y \rangle.$ Then, upon running any no-regret policy (\emph{e.g.,} \textsc{Hedge}) on this instance of experts, we have the following guarantee
%\begin{eqnarray*}
%	\sum_{\tau=1}^{t} \langle x_i(\tau), y_\tau \rangle  \geq \max_{i,y} \sum_{\tau=1}^t \langle x_i(\tau), y \rangle - O(\sqrt{t}),
%\end{eqnarray*} 
%which implies \eqref{reg-expr1}. In our problem, if the expert $(i,c)$ is sampled at time $t$, the online policy simply caches the subset of files given by $c$. For the single user case $m=1$, it is known from \citet{mukhopadhyay2022k} that the \textsc{Hedge} policy can be run in almost linear time. 
%
%\subsection{Derivation of a no-regret Online Caching Policy}
%
%We seek an online caching policy $\pi$ such that for all $y^* \in \Delta^N_k,$ it guarantees
%\begin{eqnarray*}
%	\max_{i} \sum_{\tau \leq t} \langle x_i(\tau), y^*-y_\tau \rangle = O(\sqrt{t}).
%\end{eqnarray*}
%Define $g_t^i(y) \equiv \langle x_i(t), y\rangle.$ We first consider a non-causal policy $\tilde{\pi}$ that has access to the reward functions $g^i_t$'s at the beginning of round $t$. Specifically, the action of the policy $\tilde{\pi}$ at round $t$ is given by:
%\begin{eqnarray*}
%	\tilde{y}_{t+1} = \arg \max_{y \in \Delta^N_k} \min_i \sum_{\tau=1}^t g^i_\tau(y) = \arg \max_{y \in \Delta^N_k} \sum_{\tau =1}^t g_\tau^{\tilde{i}_{t+1}}(y),
%\end{eqnarray*}  
%where $\tilde{i}_{t+1}$ be the index of a user which achieves the minimum user index in the above (ties are broken arbitrarily).   
%Now consider a standard OCO problem where the reward function at round $t$ is defined as: 
%\[f_t(y)= g^{\tilde{i}_{t+1}}_t(y).\]  
%Applying the BTL lemma to the sequence of reward functions $\{f_t\}_{t=1}^T$'s we immediately conclude that, the policy $\tilde{\pi}$ has a non-positive regret, \emph{i.e.,} for all $y^* \in \Delta^N_k,$ we have that
%\begin{eqnarray*}
%	\sum_{t=1}^T f_t(y^*)- f_t(\tilde{y}_{t+1}) \leq 0.
%\end{eqnarray*} 
%The above implies that: 
%



















==> formulation.tex <==
\section{Introduction and System Model} \label{formulation}
We consider an online problem, which we call \emph{Online Fair Caching} (OFC). In this problem, $m$ users are connected to a single cache of capacity $k$ (see Figure \ref{sys-diagram} for a schematic). At each round, every user request one file from a library of size $N.$ The file request sequence could be adversarial. At the beginning of each round $t$, an online caching policy prefetches $k$ files on the cache, denoted by the vector $y_t \in \{0,1\}^N$ such that $||y_t||_1=k.$ The set of all feasible caching configuration is denoted by $\Delta^N_k.$ 
\footnote{In the following, we consider the relaxed action where the components of any vector $y \in \Delta^N_k$ denote the corresponding inclusion probabilities. From the any relaxed action, one can derive an integral caching policy by using Madow's sampling with these probabilities. As a result, the variable $R_i(t)$'s in the regret definition are to be taken as the expected hit rates (\emph{not} the actual hits), which can be computed by the policy from the inclusion probabilities $\bm{y}_t$ as in Eqn.\ \eqref{reward-evolution}.}.  Immediately after the prefetching at round $t$, each user $i$ reveals its file request, represented by the one-hot encoded vector $x_i(t)$, $1\leq i \leq m$. A special case of the above caching model for a single user ($m=1$) has been investigated in our previous work \citep{SIGMETRICS20, paria2021, mhaisen2022optimistic, ITW22}. 

\begin{figure}[!ht]
\centering
	\includegraphics[scale=0.3]{diagram.pdf}
	\put(-35, 35){Library}
	\put(-155,35){Cache of capacity $k$}
	\put(-265,99){User $1$}
    \put(-265,64){User $2$}
    \put(-268,10){User $m$}
	\caption{System model}
	\label{sys-diagram}
\end{figure}

Let the variable $R_i(t)$ denote the cumulative hits obtained by the $i$\textsuperscript{th} user up to round $t \geq 1$. Clearly,
\begin{eqnarray} \label{reward-evolution}
	R_i(t) = R_i(t-1) + \langle x_i(t), y_t \rangle, ~~1 \leq i \leq m,
\end{eqnarray}
where $R_i(0)=1, \forall i. $ By iterating the above recursion, the variable $R_i(t)$ can be alternatively expressed as follows:
\begin{eqnarray} \label{hit-eqn}
	R_i(t) = 1+ \sum_{\tau=1}^t \langle x_i(\tau), y_t \rangle.
\end{eqnarray}
From the above, we can see that $R_i(t)$ is a function of only the first $t$ caching action variables $\{y_\tau\}_{\tau=1}^t.$ Let the utility function for any user be given by the concave function $\phi: \mathbb{R}_+ \to \mathbb{R}_+,$ where the function $\phi$ belongs to the class of all admissible utilities defined later.
Our objective is to design an online caching policy that minimizes the regret of the cumulative utilities of all users up to time $T$ compared to any offline time-invariant benchmark that caches a fixed set of $k$ files $y_t=y^*$ at all rounds $t \in [T]$, which, in turn, generates a cumulative hit-rate sequence $\{R_i^*(t)\}_{t=1}^T, 1\leq i \leq m$, \emph{i.e.,}
\begin{eqnarray} \label{regret-def}
	\min_{\{y_t\}_{t=1}^T}\mathcal{R}_T \equiv \sum_{t=1}^T \sum_{i=1}^m \phi(R_i^*(t))-  \sum_{t=1}^T \sum_{i=1}^m \phi(R_i(t)). 
\end{eqnarray}
We emphasize that, although the benchmark policy $y^*$ remains fixed, the cumulative hit rates $R_i^*(t)$ vary with time according to the adversarial dynamics \eqref{reward-evolution}. Similar utility function-based performance optimization for networks has been considered earlier in stochastic setting \citep{andrews2005optimal}.
\iffalse
\subsection{Admissible utility functions}
In practice, there could be a range of choices for the utility (also known as \emph{fairness}) function $\phi$ \footnote{Our results can be straight-forwardly generalized to time-varying utility functions $\phi_t(\cdot)$ as well.}. The utility functions could be application-specific, and most importantly, they could be \emph{transparent} to the online learner \emph{throughout} the entire time-horizon. In particular, no feedback might be available to the learner regarding its functional form or even its gradients. This should be contrasted with the usual Online Convex Optimization (OCO) framework \citep{zinkevich2003online}, where the gradient of the reward functions are revealed to the learner at the end of each round. The issue of learner not knowing the the utility function may arise from the fact that the true utility of the users may depend on the nature of the files being cached (\emph{e.g.,} whether the files contain movies or fixed datasets, or real-time data of a UAV). Furthermore, it could also be difficult to analytically characterize the true utility function. Interestingly, our proposed caching policy achieves a sublinear regret bound \emph{uniformly} for \emph{any} utility function in the class $\Phi$ up to determining a scalar hyper-parameter $0<\epsilon<1$ described later. 
%An interesting consequence of the above simple derivation is that the proposed policy $\pi$ continues to yield a sublinear regret if the utility functions satisfy some mild conditions.
%Assume that the fairness function of the $i$\textsuperscript{th} user at round $t$ be given by $\phi_i(t).$ Then, following the same line of derivation leading to \eqref{first-order-bound}, the regret, in this case, can be upper-bounded as:
%
%We now make the following assumptions on the class $\Phi$ of admissible utility functions.
We now characterize the class of all admissible utility functions in the following definition.  
\begin{framed}
\begin{definition}[(The class of admissible utility functions $\Phi$)] \label{admissible}
	The class of admissible utility functions  $\Phi$ consists of all functions $\phi : \mathbb{R}_+ \to \mathbb{R}_+$ satisfying the following two conditions:
	
	1. 	Each function $\phi \in \Phi$ is non-decreasing, differentiable, and concave.
	
	2. $J_\phi(T)\equiv \int_{0}^T \sqrt{x} \phi'(x) dx = o(T), \forall \phi \in \Phi.$
\end{definition}
\end{framed}
%\begin{assumption}
%
%\end{assumption}
%	%\item  for each user $i \in [m]$.
%	\begin{assumption}
%			$J(T)\equiv \int_{1}^T \sqrt{x} \phi_i'(x) dx = o(T).$
%	\end{assumption}
% 
%\end{enumerate}
%\end{framed}
Upon integrating by parts, Condition 2 can also be given an alternative characterization. Note that
\begin{eqnarray*}
	\int_1^T \sqrt{x} \phi'(x) dx = \sqrt{T}\phi(T) - \frac{1}{2}\int_{1}^T \frac{\phi(x)}{\sqrt{x}} dx.    
\end{eqnarray*}

Thus Condition 2 is equivalent to the following condition:
\begin{eqnarray*}
	\overline{g(T)} \geq  2 g(T)- o(1),
\end{eqnarray*}
where $g(x) \equiv \frac{\phi(x)}{\sqrt{x}},$ and the term on the left denotes the average value of the function $g$ in the interval $[0,T].$ 

\textbf{Examples:}  Many common utility functions used in practice are included in the admissible class $\Phi.$ This includes the logarithmic utility function $\phi_{\textrm{logarithmic}}(x)=\log(x)$, and $\alpha$-fair utility functions  $\phi_\alpha(x) = \frac{x^{1-\alpha}}{1-\alpha}$, where $\nicefrac{1}{2}<\alpha \leq 1.$ The integral $J_\phi(\cdot)$ for these classes of functions can also be easily evaluated in closed-form. 

%\subsubsection*{Closed-form expressions of the integral $J (\cdot)$ for common utility functions}
%\textbf{Case 1: Logarithmic Utility}

1. In the case of the logarithmic utility function, we have $\phi_{\textrm{logarithmic}}(x) = \log (x). $ Hence, 
\begin{eqnarray} \label{log-J}
	J_{\textrm{logarithmic}}(T) = \int_{0}^T \frac{\sqrt{x}}{x} dx = 2T^{\nicefrac{1}{2}},   
\end{eqnarray}
 which can be seen to be sublinear. 
 
 2. In the case of $\alpha$-fair utility, we have $\phi_\alpha(x)= \frac{x^{1-\alpha}}{1-\alpha},$ for some $0<\alpha<1.$ Hence,
 \begin{eqnarray} \label{J-alpha}
 	J_{\alpha-\textrm{fair}}(T) = \int_{0}^T \sqrt{x} \frac{1}{x^\alpha} dx = \frac{1}{3/2-\alpha}T^{3/2 - \alpha}.
 \end{eqnarray}
 It can be seen from the above expression that $J_\alpha(T)$ is sublinear as long as $\frac{1}{2}<\alpha <1.$
 

%\textbf{Note:} 1. The above result holds even for a sequence of time-varying utility functions $\{\phi_t()\}_{t \geq 1}$ satisfying the conditions. 

To recap, the Online Fair Caching problem has the following information structure- (1) The utility function $\phi \in \Phi$ remains unknown to the learner throughout. (2) The file requests $x_i(t), i \in [m]$ for round $t$ is revealed to the learner only after the caching decision $y_t \in \Delta^N_k$ is made for round $t$.   
\fi

\subsection{On the non-triviality of the OFC problem}

We now outline the fundamental difference between the OFC problem \eqref{regret-def} and the usual Online Convex Optimization (OCO) problem \citep{hazan2019introduction}. In the standard OCO problem, the reward accrued at any round $t$ depends on the action taken on round $t$ \emph{only}. In particular, the OCO framework applies to the  \emph{memoryless} systems where the action taken at a round does not affect the reward functions seen in the subsequent rounds. On the other hand, in the OFC problem, the caching action $\bm{y}_t \in \Delta^N_k$ taken at round $t$ affects \emph{all} future rewards through the cumulative hit vector $\bm{R}(t)$. For the same reason, recent online algorithms developed for systems with \emph{bounded memory} \citep{anava2015online} do not apply to the OFC problem. From a high-level perspective, the online fair caching problem is an instance of an adversarial Reinforcement Learning problem, for which no general algorithmic methodology is known to yield a sublinear regret. One of the surprises of this paper is that the OFC problem can be efficiently solved by making use of Online Convex Optimization subroutines with \emph{perturbed} requests even when the utility functions are unknown. 

\section{Preliminaries} \label{prelims}
In this section, we recall some recent adaptive regret bounds achieved by OGD-like algorithms. The $L_p$-deviation of a sequence of reward function $\{f_t\}_{t=1}^T$ is defined as
\begin{eqnarray*}
	D_p= \sum_{t=1}^T \max_{x \in X} || \nabla f_t(x) - \nabla f_{t-1}(x)||_p^2. 
\end{eqnarray*}
The paper \cite{chiang2012online} proves the following static regret bound for the OEGD algorithm proposed in that paper:
\begin{theorem}[\cite{chiang2012online}] \label{adaptive-regret}
	When the $L_2$-deviation of the loss function is $D_2$, the regret of the OEGD algorithm is at most $O(\sqrt{D_2}).$
\end{theorem}


\section{Policy design} \label{analysis}
Our central idea is to reduce the OFC problem to an instance of online linear optimization problem, which can be solved with the standard OCO techniques \citep{SIGMETRICS20, mukhopadhyay2022k}. In doing so, it turns out that one also needs to slightly perturb the input request sequence itself to make the reduction work.


Using the fact that $\phi(R_i(t))$ is a concave function of the previous action variables $\{y_{\tau}\}_{\tau=1}^t,$ using the first-order Taylor series bound, we can write 
\begin{eqnarray} \label{first-order-bound}
	\phi(R_i^*(t)) - \phi(R_i(t)) \leq  \phi'(R_i(t)) \sum_{\tau=1}^t \langle x_i(\tau), y^*-y_\tau \rangle.  
\end{eqnarray}
Hence, summing up the above inequality, we can upper bound the regret of any online caching policy as follows:  
\begin{eqnarray} \label{regret-expr3}
	\textrm{Regret}_T \leq \sum_{i=1}^m \sum_{t=1}^T \phi'(R_i(t))\bigg(\sum_{\tau \leq t} \langle x_i(\tau), y^*-y_\tau \rangle \bigg).
\end{eqnarray}

\section{Design of a No-regret Policy}
Assume that the cache capacity $k$ is no less than the number of users $m$ in the system. In this setup, we now design a no-regret policy for the logarithmic utility function against a much stronger comparator sequence $\pi^*=\{y^*_\tau\}_{\tau \geq 1}$ which, at each round $t$, caches all files requested by the users, \emph{i.e.,} $y^*_\tau = \bigvee_{i} x_i(\tau),$ where the $\bigvee$ operation is applied component wise. Clearly, the offline policy $\pi^*$ achieves the maximum utility over a time horizon, with $R_i(t) =t, \forall i,t.$ This yields the following optimal value for the offline cumulative utility function: 
\begin{eqnarray*}
	\textsc{Obj}^* = m \sum_{t=1}^T \log t \stackrel{\textrm{(Stirling)}}{\approx} m \bigg(\frac{1}{2}\log(2\pi T) + T \ln T -T \bigg) \approx mT\ln T.    
\end{eqnarray*}
We now design an online policy that achieves a sublinear regret with respect to this benchmark. Adapting the regret bound \eqref{regret-expr3} to the setting of time-varying benchmark, we have 
\begin{eqnarray} \label{regret-bound4}
	\textrm{Regret}_T \leq \sum_{i=1}^m \sum_{t=1}^T \frac{1}{R_i(t)}\bigg(\sum_{\tau \leq t} \langle x_i(\tau), y_\tau^*-y_\tau \rangle \bigg).
\end{eqnarray}
Note that since the offline policy $\pi^*$ always scores a cache hit for all users, the inner-product is always non-negative, no matter what action sequence $\{y_\tau\}_{\tau \geq 1}$ the online policy takes. Since the cumulative hits $R_i(t)$ is a monotone non-decreasing function for all users under the action of any caching policy, we have $R_i(\tau) \leq R_i(t), \forall \tau \leq t.$ Hence, we can further upper bound the regret from \eqref{regret-bound4} as: 
\begin{eqnarray} \label{reg-bd5}
	\textrm{Regret}_T \leq \sum_{t=1}^T \underbrace{\bigg(\sum_{\tau=1}^t\langle \sum_{i=1}^m \frac{x_i(\tau)}{R_i(\tau)}, y^*_\tau - y_\tau \rangle \bigg)}_{\textrm{OLO}}. 
\end{eqnarray}  
The term within the braces is the dynamic regret of the online policy corresponding to the offline action sequence $\pi^* \equiv \{y^*_\tau\}_{\tau \geq 1}.$ Now as shown in \ref{hit-rate-lb}, the OEGD policy automatically ensures that $R_i(t) = \Omega(\frac{t}{\log t}).$ Hence, the gradient variation for the OLO problem shown in \eqref{reg-bd5} can be bounded as 
\begin{eqnarray*}
	V_t = \sum_{\tau=2}^t || \sum_{i} \frac{x_i(\tau-1)}{R_i(\tau-1)} - \sum_{i} \frac{x_i(\tau)}{R_i(\tau)} ||_2^2 = O(\sum_{\tau} \frac{\log^2 \tau}{\tau^2}) = O(1),
\end{eqnarray*}
where the last equality follows from the fact that $\int_{1}^\infty \frac{\log^2 x}{x^2} dx =2 < \infty.$
Hence, the OEGD policy \citep[Theorem 1]{zhao2020dynamic} achieves a dynamic regret bound of $O(\sqrt{1+ P_t})$.  Hence, assuming 
\[ \sum_{t=1}^T \sqrt{1+P_t} = o(T \log T), \]
the proposed policy asymptotically achieves the optimal objective value. 

\iffalse
\section{Static Regret of the Online Policy }
We now return to the case of static regret where the offline caching configuration $y^*$ remains fixed in time. Now, for each $i, t,$ we define two exhaustive and mutually exclusive  events: 
\begin{eqnarray*}
	G_{i,t} = \langle x_i(\tau), y^*-y_\tau \rangle < 0, \\
	B_{i,t} = \langle x_i(\tau), y^*-y_\tau \rangle \geq 0.
\end{eqnarray*}
Intuitively, on occurence of the event $G_{i,t},$ the online policy does strictly better than the offline static benchmark in terms of scoring cache hits for the $i$\textsuperscript{th} user on round $t$. On the other hand on occurrence of the event $B_{i,t}$ the benchmark does at least as good as the online policy in terms of scoring a cache hit on the $i$\textsuperscript{th} user. Then we can express the above regret upper bound as:
\begin{eqnarray*}
	\textrm{Regret}_T &\leq& \sum_{t=1}^T \sum_{i=1}^m \frac{1}{R_i(t)} \bigg(\sum_{\tau \leq t} \langle x_i(\tau), y^*-y_\tau \rangle \bigg) (\mathds{1}(B_{i,\tau}) + \mathds{1}(G_{i,\tau})) \\
	& \leq & \sum_{t=1}^T \bigg( \sum_{\tau \leq t} \langle \sum_{i=1}^m \frac{x_i(\tau)}{R_i(\tau)}, y^*-y_\tau \rangle \mathds{1}(B_{i,\tau}) \bigg)
\end{eqnarray*}

\fi













 
\section{Lower bound to Hit Rates under a No-regret Policy} \label{hit-rate-lb}

\begin{theorem}
	The OEGD Policy achieves $O(1)$ static regret and ensures that $R_i(t) \geq \Omega(\frac{t}{\log t}), \forall i, t.$
\end{theorem}

In this section, we establish that the OGD policy achieves $O(1)$ regret for the logarithmic utility function and simultaneously achieves almost linearly many hit rates for all users. 
%the causal online caching policy that solves a causal version of the OLO problem \eqref{olo-red} with $w_i(\tau) \gets \frac{1}{R_i(\tau)}, \forall i$ scores almost linearly many cache hits with respect to time for each user. 
%The causal OCO policy with the above rate can also be seen to be an instance of a \emph{Proportional Fair} policy, that prioritizes the users in inverse proportion to their current hit rates. 
For this, let us first recall the standard data-dependent worst-case static regret bound for an OCO policy with adaptive learning rates \citep[Theorem 4.14]{orabona2019modern}, \citep{zhao2020dynamic}:
\begin{eqnarray*}
	\reg = O\bigg(\sqrt{\sum_{t=1}^T ||\bm{g}_t||_2^2}\bigg)
\end{eqnarray*}
where $||\bm{g}_t||_2$ denotes the $\ell_2$ norm of the reward function at round $t$. In our case, the above theorem yields 
\begin{eqnarray} \label{adaregret}
	\reg = O(\sqrt{\sum_{t=1}^T\sum_i \frac{1}{R_i^2(t)}}).
\end{eqnarray}


By virtue of the sublinear regret property of the OCO policy, for any fixed caching configuration $y^*,$ we have for any time step $T$: 
\begin{eqnarray} \label{reg-ineq}
	\sum_{t=1}^T \sum_{i} \langle \frac{x_i(t)}{R_i(t)}, y_t \rangle  \geq \sum_{t=1}^T \sum_i \langle \frac{x_i(t)}{R_i(t)}, y^* \rangle - \reg, 
\end{eqnarray} 
where $\reg$ denotes the cumulative regret of the causal OCO policy up to time $T$. Since the cumulative hits of each user is monotonically non-decreasing, we have:
\begin{eqnarray} \label{bd0}
	R_i(T) \geq 1, \forall i.
\end{eqnarray}
This yields the our first upper-bound for the regret of the OLO problem:
\begin{eqnarray} \label{reg-bd1}
	\reg = O(\sqrt{T}).
\end{eqnarray}

We will now strengthen the above upper-bound using a novel \emph{bootstrapping} method, which \emph{simultaneously} tightens the lower bound for the cumulative hits \eqref{bd0} and improves the regret upper bound \eqref{reg-bd1}. 
%\newpage
\iffalse
\hrule
\textbf{Note} The actual regret bound could be better than $O(\sqrt{T}).$ Because if the $R_i(T)'s$ increase linearly, then the magnitude of the gradients increase linearly as well. Upon using the regret bound in terms of the gradients, this yields an $O(1/\sqrt{T})$ regret bound for large $T$. 
\hrule
 \fi
 
 
Since $\langle x_i(t), y_t \rangle = R_i(t+1)-R_i(t),$ inequality \eqref{reg-ineq} yields: 
\begin{eqnarray} \label{oco-prop}
	\sum_i \log R_i(T) = \sum_i \int_{1}^{R_i(T)} \frac{dR_i(t)}{R_i(t)} 
	\geq  \sum_i \sum_{t=1}^T \frac{R_i(t+1)-R_i(t)}{R_i(t)} \geq   \sum_i \frac{\textsf{OPT}_i(T)}{R_i(T)} - \reg, 
\end{eqnarray}
where we have used the fact that the cumulative hits $R_i(t)$'s are monotone non-decreasing and $\textsf{OPT}_i(T)$ denotes the cumulative hits of the $i$\textsuperscript{th} user obtained by any fixed offline policy $y^*.$ Recall that inequality \eqref{oco-prop} is valid for any fixed caching configuration $y^* \in \Delta^N_k$. Hence, taking uniform average over all fixed cache configurations obtained by randomly selecting each item with uniform probability, we have that \[\textsf{OPT}_i(T) \geq \beta T, \forall i\] for $\beta \equiv \frac{k}{N}>0.$  Hence, the OEGD policy yields the following performance bound:
\begin{eqnarray} \label{func-ineq1}
	\frac{1}{T} \sum_i \log R_i(T) \geq \beta \sum_i \frac{1}{R_i(T)} - \frac{\reg}{T}.
\end{eqnarray}
Since $0<R_i(T) \leq T, \forall i,$ the above inequality yields for any user $i \in [m]$:
\begin{eqnarray*}
	\frac{m \log T}{T} \geq \frac{\beta}{R_i(T)} - \frac{\reg}{T}. 
\end{eqnarray*}
\emph{i.e.},
\begin{eqnarray*}
	\frac{\reg + m \log T}{T} \geq \frac{\beta}{R_i(T)}.
\end{eqnarray*} 

Now, since from Eqn.\ \eqref{reg-bd1}, we have, $\reg = O(\sqrt{T}),$ the previous estimate yields:
\begin{eqnarray} \label{bd1}
	R_i(T) = \Omega(\sqrt{T}).
\end{eqnarray}
This implies that the difference between two successive gradients is 
\begin{eqnarray*}
	 ||\sum_i \frac{x_i(t)}{R_i(t)} - \sum_i \frac{x_i(t-1)}{R_i(t-1)}||_2 \stackrel{\textrm{(Triangle ineq.)}}{\leq} \sum_i O(\frac{1}{\sqrt{t}})= O(\frac{1}{t^{1/2}}).
\end{eqnarray*}
Upon combining \eqref{adaregret} with the new lower bound \eqref{bd1} for the cumulative hits, and using Theorem \ref{adaptive-regret}, we can now boost the previous regret bound \eqref{reg-bd1} to arrive at the following tighter bound: 
\begin{eqnarray} \label{reg-bd2}
	\reg = O\bigg(\sqrt{\sum_{t=1}^T} \frac{1}{t}\bigg)= O(\sqrt{\log T}).
\end{eqnarray}
Substituting the new regret bound in \eqref{func-ineq1}, we arrive at the following lower bound for cumulative hits:
\begin{eqnarray*}
	R_i(T) = \Omega\big(\frac{T}{\log T}\big), \forall i. 
\end{eqnarray*} 
Using the regret bound \eqref{adaregret} one more time, we have the following final upper bound on regret
\begin{eqnarray*}
	\textrm{Reg}(T) = O(\sqrt{\sum_{t=1}^T \frac{(\log t)^2}{t^2}})=O(1). 
\end{eqnarray*}

\section{An Alternative Reward Structure}
We consider the reward only at the end of the horizon, \emph{i.e.,} the regret of a policy is defined as
\begin{eqnarray*}
	\textrm{Reg}(T) \equiv \sum_i \phi (R_i^*(T)) - \sum_i \phi (R_i(T)),
\end{eqnarray*}
where $\phi$ is some non-decreasing concave function. Note that, we recover the cumulative hit rate maximization problem by taking the utility function $\phi$ to be $\phi(x)=x.$ We want to design a policy with a non-trivial regret bound. 



%Note that the weight $w_i(\tau)$ can be alternatively expressed as $w_i(\tau) = \sum_{t=1}^T \frac{1}{R_i(t)} - \sum_{t=1}^{\tau-1} \frac{1}{R_i(t).}$ In this expression, the first term is unknown but the second term is known at time $\tau.$ We can either use the principle of optimism in the face of uncertainty or doubling trick to estimate the quantities $w_i(\tau)$ and run an OLO policy to guarantee an $O(\sqrt{T})$-regret. 


%\subsection{A Naive Policy}
%Since the cumulative hits of each user are non-decreasing with time, we have the following crude estimate $w_i(\tau) \leq \frac{T-\tau+1}{R_i(\tau)-1}, \forall i.$ Hence, the problem \eqref{olo-red} corresponds to an online linear optimization problem where the reward vector at step $\tau$ is given by 
%\begin{eqnarray*}
%	\bm{g}_\tau = (T-\tau+1)\sum_{i} \frac{\bm{x}_i(\tau)}{R_i(\tau)-1}. 
%\end{eqnarray*}
%In principle, it is possible to design an online caching policy using the framework designed in \cite{mukhopadhyay2022k}. 
%However, since the gradients can not be bounded reasonably, the usual analysis fails to yield a sublinear regret bound. 

%\subsection{A No-regret fair caching policy}
%Let's now make the assumption that the hit rates of the users converge under the action of the given policy. In other words, 
%Clearly, the weight vector $\bm{w}(\tau)$ at time $\tau$ depends on the future file request sequence from the users, and, as such, the problem \eqref{regret-def} is \emph{not} an instance of the standard OCO problem. On the other hand, we make the critical observation that if the weights can be appropriately controlled under the action of a given online policy, the problem \eqref{regret-def} can be reduced to a standard OCO problem. In the following, we consider a causal OCO policy that simply ignores all future terms in the weight function. 
%Towards this, we confine our attention to the class of online caching policies $\Pi_{\bm{\alpha}}$ where
%\begin{eqnarray} \label{rate-constraint}
%	w_i(\tau) = O(\ln (T)). 
%\end{eqnarray} 
%there exist strictly positive numbers $\{\alpha_i\}_{i=1}^m$ with $0<\alpha_i\leq 1, \forall i,$ s.t. w.h.p. 
%\begin{eqnarray} \label{rate-constraint}
%	 \frac{R_i(t)}{t} \geq  \alpha_i, ~~ \forall i,t . 
%\end{eqnarray} 
%where the expectation is taken with respect to the randomness of the policy. 
\iffalse
\subsection{A class of policies guaranteeing constraint \eqref{rate-constraint}}
%Note that \eqref{rate-constraint} is not a very restrictive assumption as an 
Consider a randomized caching policy $\pi$ that, at every round, caches $C$ files uniformly at random with probability $\epsilon,$ and runs some other online caching policy $\pi^{\textrm{OCO}}$ (to be described later) with probability $1-\epsilon.$ Since the cumulative hits $R_i(t)$'s are non-decreasing with time, the following theorem shows that the policy $\pi$ satisfies the constraint \eqref{rate-constraint} with some admissible $\bm{\alpha},$ irrespective of the policy $\pi^{\textrm{OCO}}.$ The proof is deferred to the Appendix.

%\begin{appendixproof}
%Proof of the theorem.	
%\end{appendixproof}
%
%\begin{theoremrep}
\begin{theorem}
The randomized policy $\pi$ guarantees constraint \eqref{rate-constraint} w.h.p. 
%\end{theoremrep}
\end{theorem}
For any fixed $0\leq \delta <1$ and starting from any round $\tau,$
divide the remaining rounds into successive \emph{frames} where each frame consists of consecutive $\lambda$ rounds. We make the following claim:
\begin{proposition} \label{hit-prop}
	Upon setting the frame length $\lambda \equiv \frac{1}{\epsilon C/N}\ln (m/\delta),$ in any future frame, all users receive at least one cache hit with probability at least $1-\delta.$
\end{proposition}

\begin{proof}
Note that \emph{irrespective} of the particular file requested (which could be adversarial), due to the randomized exploration, on every round, each user receives a cache hit with probability at least $\epsilon C/N.$
	 Now, for any user $i$, let $\mathcal{E}_{i}$ be the event denoting that the $i$\textsuperscript{th} user receives at least one hit in any given future frame. Then we have:
	\begin{eqnarray*}
		\mathbb{P}(\mathcal{E}_{i}^c) \leq \bigg(1- \epsilon \frac{C}{N}\bigg)^\lambda \leq e^{-\epsilon \lambda C/N}.  
	\end{eqnarray*}
Hence,
	\begin{eqnarray*}
		\mathbb{P}(\cap_{i=1}^m \mathcal{E}_{i})=1- \mathbb{P}(\cup_{i=1}^m \mathcal{E}^c_{i}) \stackrel{(a)}{\geq} 1-me^{-\epsilon \lambda  C/N} \stackrel{(b)}{\geq} 1-\delta,
	\end{eqnarray*}
	where in (a) we have used the union bound and (b) follows upon setting $\lambda = \frac{1}{\epsilon C/N}\ln (m/\delta).$ 
	\end{proof}
	
	%The above implies that \emph{all} users receive at least one cache hit in every frame with probability at least $1-\delta.$ 
	Let $\{\mathcal{F}_j\}_{j=1}^T$ be the natural filtration generated by the policy. We now make the following claim:
	\begin{proposition} \label{hp-bound}
	On any round $\tau,$ we have
	  \[\mathbb{P}\bigg[\frac{1}{R_i(\tau)} \leq w_i(\tau) \leq \frac{\lambda}{R_i(\tau)} + \ln\big(1+T\big), \forall i \bigg|\mathcal{F}_{\tau-1}\bigg] \geq 1-\frac{\delta T}{\lambda},\] where the parameter $\lambda$ was chosen as in Proposition \ref{hit-prop}.
	\end{proposition}
	\begin{proof}
	Recall that 
	\begin{eqnarray*} 
			 w_i(\tau) = \sum_{t=\tau}^T \frac{1}{R_i(t)},
	\end{eqnarray*}
	from which the first bound follows immediately. 
 Let $t_j$ denote the index of the first round of the subsequent $j$\textsuperscript{th} frame with $t_1=\tau$. Since the variables $\{R_i(t)\}_t$ are non-decreasing, we can upper-bound $w_i(\tau)$ as 
	\begin{eqnarray} \label{weight-def}
		w_i(\tau) \leq \lambda \sum_{j=1}^{\frac{T-\tau}{\lambda}} \frac{1}{R_i(t_j)}.
	\end{eqnarray}
	From Proposition \ref{hit-prop} and using a union bound over all subsequent frames, we have with probability at least $1- \delta (T-\tau)/\lambda \geq 1-\frac{\delta T}{\lambda}:$
	\begin{eqnarray*}
		R_i(t_j) \geq R_i(\tau) + j-1, ~~ \forall i,j.
	\end{eqnarray*}
	Hence, with probability at least $1-\nicefrac{\delta T}{\lambda}$ conditioned on the past, the weight \eqref{weight-def} can be upper bounded as 
	\begin{eqnarray*}
		w_i(\tau)&\leq& \lambda \sum_{j=1}^{\frac{T-\tau}{\lambda}} \frac{1}{R_i(\tau)+j-1} \\
		&\leq& \frac{\lambda}{R_i(\tau)} + \lambda  \int_{0}^{\frac{T-\tau}{\lambda}} \frac{dx}{R_i(\tau)+ x} \\
		&=& \frac{\lambda}{R_i(\tau)}+ \lambda \ln \bigg(1+ \frac{T-\tau}{\lambda R_i(\tau)}\bigg)\\
		&\leq& \frac{\lambda}{R_i(\tau)}+ \lambda \ln T~~ \forall i.
	\end{eqnarray*}
	where the last inequality follows from the fact that $\lambda \geq 1, R_i(\tau) \geq 1, \forall i, \tau \geq 1,$ and the monotonicity of the cumulative hits.
	\end{proof}
	
	%The above result readily yields an upper bound on the conditional expectation of the weight vector at time $\tau.$
Using a union bound once again, Proposition \ref{hp-bound} implies that with probability at least $1-\frac{\delta T^2}{\lambda},$ the regret bound \eqref{olo-red} can be further upper-bounded as:
\begin{eqnarray*}
	\mathcal{R}_T \leq \sum_{\tau=1}^T \langle \sum_{i} x_i(\tau) w_i(\tau), y^*- y_\tau \rangle,
\end{eqnarray*}

%as shown below. 
%, the condition \eqref{rate-constraint} can be ensured if at each round, with a small probability $\epsilon,$ we play the policy $\pi^{\textsc{RAND}},$ and with the complementary probability, we play any other online caching policy. 

%For large $\tau,$ a rough estimate for $\alpha_i$ is given by $\frac{R_i(\tau)}{\tau}.$ (To get rid of the expectations, the exploration can also be done on deterministic rounds. The regret bound should not change by more than a constant factor.)
%With this assumption, we have the following upper bound for the weight function
%\begin{eqnarray*}
%	w_i(\tau) \leq \frac{\tau}{R_i(\tau)} \sum_{t=\tau}^T \frac{1}{t} \leq \frac{\tau \ln (T/\tau)}{R_i(\tau)} \leq \frac{\ln(T)}{R_i(\tau)/\tau}.
%\end{eqnarray*}
%This yields $w_i(\tau)= O(\frac{\ln T}{\alpha_i}).$ 
Hence, the online fair caching problem reduces to an OLO problem with the following reward vector at time $\tau:$ 
\begin{eqnarray*}
	\bm{g}_\tau = \ln(T) \sum_i \frac{\bm{x}_i(\tau)}{R_i(\tau)/\tau}.
\end{eqnarray*}
The above is the same as the online caching problem where the cache-hits are discounted by the current hit-rates, inducing fairness among the users. 
Since $|| \bm{g}_\tau||_2 \leq \ln(T)(\sum_{i}\frac{1}{\alpha_i})$, using the online caching policy described in \cite{mukhopadhyay2022k}, we get the following sublinear regret guarantee:
\begin{eqnarray*}
	\mathcal{R}_T \leq 2\frac{\ln T}{\epsilon} (\sum_i \frac{1}{\alpha_i})\sqrt{2CT\ln \frac{N}{C}} + \epsilon m T \ln T,
\end{eqnarray*} 
where the last term is an upper bound on the expected regret incurred due to the uniform exploration. By optimizing over $\epsilon,$ we get a policy with $\tilde{O}(T^{3/4})$ regret. 

\textbf{TODO} 
\begin{enumerate}
	\item It is probably unnecessary to do uniform exploration to ensure the constraint \eqref{rate-constraint}. I think, the policy $\pi^{\textrm{OCO}}$ does sufficient exploration on its own to ensure \eqref{rate-constraint}. If we can get rid of the exploration part, we will have a policy with $O(\sqrt{T})$ regret. 
	\item Also, it would be interesting to carry out the above analysis for $\alpha-$fair utility functions.
	\item After proving the sublinear regret bound, we may iterate the regret bound again to obtain tighter bounds for $\vec{\bm{\alpha}}.$
	\item  Strengthening of Theorem 1 using Doob-Kolmogorov Maximal inequality.
\end{enumerate}


\subsection{Observation-I}
%By switching the order of summations, the regret upper bound \eqref{olo-red} can be alternatively expressed as :
Recall that from Eqn.\ \eqref{first-order-bound}, the regret for any policy can be bounded as:
\begin{eqnarray} \label{regret-expr2}
	\textrm{Regret}_T \leq \sum_{i=1}^m \sum_{t=1}^T \frac{1}{R_i(t)} \bigg(\sum_{\tau \leq t} \langle x_i(\tau), y^*-y_\tau \rangle \bigg).
\end{eqnarray}
The inner summation is simply the regret of a policy up to round $t$ for the linear hit-rate maximization problem $\mathcal{P}'$ for the $i$\textsuperscript{th} user. 

\fi 
%
%Now suppose that we can come up with an adaptive caching policy $\pi$ which ensures sublinear regret for each users, \emph{i.e.,} for all $y^* \in \Delta^N_k,$ for all time $t \geq 1,$ and all users $i,$ we have:  
%\begin{eqnarray} \label{reg-expr1}
%	\sum_{\tau \leq t} \langle x_i(\tau), y^*-y_\tau \rangle = O(\sqrt{t}). 
%\end{eqnarray} 
%\begin{lemma} \label{rate-lb}
% Under the above policy $\pi,$ for all users $i \in [m],$ we have $R_i(t) \geq \frac{k}{N}t - O(\sqrt{t}), \forall t \geq 1. $
%\end{lemma}
%\begin{proof}
%	Since the regret bound \eqref{reg-expr1} is valid for all $y^* \in \Delta^N_k,$ we have 
%	\begin{eqnarray*}
%		R_i(t)= \sum_{\tau \leq t} \langle x_i(\tau), y_\tau \rangle \geq \sum_{\tau \leq t} \langle x_i(\tau), y^* \rangle - O(\sqrt{t}).
%	\end{eqnarray*}
%	Now taking the uniform average of the RHS over all feasible $y^*,$ we have: 
%	\begin{eqnarray*}
%		R_i(t) \geq \frac{k}{N}t - O(\sqrt{t}).
%	\end{eqnarray*}
%\end{proof} 
%Hence, under the action of the policy $\pi,$ the regret for the original problem can be upper-bounded from \eqref{regret-expr2} as follows:
%\begin{eqnarray*}
%		\textrm{Regret}_T \leq \sum_{i=1}^m \sum_{t=1}^T \frac{O(\sqrt{t})}{\nicefrac{kt}{N}- O(\sqrt{t})} \leq \sum_{i=1}^m \sum_{t=1}^T O(\frac{1}{\sqrt{t}}) = O(\sqrt{T}).
%\end{eqnarray*}
%\subsection{Observation-II}
%
%Using Lemma \ref{rate-lb}, the regret of the policy $\pi$ can be upper bounded as 
%\begin{eqnarray*}
%	\textrm{Regret}_T \stackrel{(a)}{\leq} \sum_{i=1}^m \sum_{t=1}^T O(\sqrt{t})\phi_i' \big(\nicefrac{kt}{N}-O(\sqrt{t}) \big) = O\big(\sum_{i} \int_{1}^T \sqrt{t}\phi'_i(t) dt\big) \stackrel{(b)}{=}  o(T), 
%\end{eqnarray*}
%where inequality (a) follows from Assumption (1) and equality (b) follows from Assumption (2). 
%
\iffalse
\subsection{Designing a No-Regret Fair Caching Policy with Perturbed Requests}
%In this Section, let us denote the file requested on round $t$ by the $i$\textsuperscript{th} user by $z_i(t),  i\in [m], t \in [T].$ 
Fix a small perturbation probability $0 < \epsilon <1,$ to be fixed later \footnote{We will see that $\epsilon \to 0$ as $T \to \infty$.}. Let $\{U_i(t)\}_{t=1}^T$ be a sequence of i.i.d. random variables such that each r.v. is distributed uniformly on the library $[N]$\footnote{$U_i(t)$ can also be replaced by its expectation, \emph{i.e.,} the deterministic vector $\nicefrac{k}{N} \mathds{1}_N$.} Next, for each request sequence $\{x_i(t)\}_{t=1}^T,$ we derive a new perturbed sequence $\{\hat{x}_i(t)\}_{t=1}^T$ as follows:
\begin{eqnarray*}
\hat{x}_i(t) =	\begin{cases}
	 x_i(t), ~~\textrm{w.p.}~~ 1-\epsilon\\
	 U_i(t), ~~\textrm{w.p.}~~ \epsilon. 	
	\end{cases}
\end{eqnarray*}
In our proposed policy, the online learner is fed with the perturbed request sequence $\{\hat{x}_i(t)\}_{t \geq 1}.$  In the following, we will see that the perturbation makes the design and analysis of a no-regret fair caching policy significantly easier. Although, our motivation for perturbing the original request sequence is to aid designing a no-regret policy, the perturbation may also be necessary if the request sequence need to protect the privacy of the users. In this case, the parameter $\epsilon$ is determined by the Differential privacy requirements of the users. 

For the perturbed request sequence $\{\hat{x}_i(t)\}_{t \geq 1},$ the probability of any user receiving a cache hit under any caching policy at any given round is at least $\frac{\epsilon k}{N}.$ Hence, w.h.p. it holds that $\hat{R}_i(t) \geq \frac{\epsilon kt}{N},$ where $\hat{\bm{R}}(t)$ denotes the cumulative hits of all users for the perturbed request sequence. Now consider a \emph{strongly adaptive} online caching policy $\pi$ that achieves $O(\sqrt{t})$ regret for all time $t \in [T],$ where the objective is to maximize the cumulative hits of all users. Hence, the regret upper bound \eqref{regret-expr3} with respect to the \emph{perturbed} file requests can be further upper-bounded as 
\begin{eqnarray*}
	\hat{\textrm{Regret}}_T &\leq& \sum_{t=1}^T \phi'(\epsilon kt/N) \bigg(\sum_{\tau \leq t} \langle \sum_{i} \hat{x}_i(\tau), y^* - y_\tau \rangle \bigg) \\
	&\stackrel{(a)}{=}& O\bigg(\sum_{t=1}^T \sqrt{t} \phi'(\epsilon kt/N) \bigg) \\
	&=& O\bigg( \int_{0}^T \sqrt{t} \phi'(\epsilon kt/N) dt\bigg) \\
	&=& O\bigg( \big(\frac{N}{k \epsilon}\big)^{3/2} \int_{0}^{\epsilon kT/N} \sqrt{x} \phi'(x) dx \bigg)\\
	&\stackrel{(b)}{=}& O\bigg( \big(\frac{N}{k\epsilon} \big)^{3/2} J_\phi\big(\frac{\epsilon k T}{N}\big) \bigg), 
\end{eqnarray*} 
where (a) follows from the property of the no-regret caching policy $\pi,$ and the function $J_\phi$ appearing in (b) has been defined in Condition 2 in Definition \ref{admissible}. 
Clearly, since the function $J(\cdot)$ is sublinear in its argument, the regret of the policy $\pi$ with the perturbed request sequence $\{\hat{\bm{x}}(t)\}_{t \geq 1}$ remains sublinear. 

\begin{algorithm}
\caption{\texttt{OFC} Policy}
\label{uncoded_inelastic}
\begin{algorithmic}[1]

\FOR {$t=1$ to $T$}
\STATE Run a strongly adaptive caching policy (\emph{e.g.,} OGD) to decide the caching configuration $y_t$ for round $t$ that yields a sublinear regret for the OLO problem with per round reward function $q_t(y_t) \equiv \langle \sum_{i=1}^m \hat{x}_i(\tau), y_\tau \rangle .$
\STATE Randomly perturb the file request of each user with probability $\epsilon$ as shown below 
\begin{eqnarray*}
\hat{x}_i(t) =	\begin{cases}
	 x_i(t), ~~\textrm{w.p.}~~ 1-\epsilon\\
	 U_i(t), ~~\textrm{w.p.}~~ \epsilon. 	
	\end{cases}
\end{eqnarray*}
  \ENDFOR
\end{algorithmic}
\end{algorithm}


\textbf{Note:} It is interesting to note that the idea of  perturbing the request sequence is akin to the concept of \emph{smoothed analysis}, where an input instance to an algorithm is randomly perturbed to guarantee an efficient run-time \citep{spielman2004smoothed}.   

\subsection{Regret with respect to the un-perturbed requests}
Now we bound the regret of the above online policy with respect to the original un-perturbed file request sequences. Let $\hat{R}_i(t)$ and $R_i(t)$ denote the number of hits received by the $i$\textsuperscript{th} user up to time $t$ for the perturbed and true sequence respectively. We can write 
\begin{eqnarray*}
	R_i(t) = \sum_{\tau=1}^t \langle x_i(\tau), y_\tau \rangle, ~~ 
	\hat{R}_i(t) = \sum_{\tau=1}^t \langle \hat{x}_i(\tau), y_\tau \rangle. 
\end{eqnarray*} 
Hence,
\begin{eqnarray*}
	\hat{R}_i(t) - R_i(t) = \sum_{\tau=1}^t \langle \hat{x}_i(\tau)-x_i(\tau), y_\tau \rangle \leq \sum_{\tau=1}^t \langle \hat{x}_i(\tau), y_\tau \rangle \mathds{1}(\hat{x}_i(\tau)\neq x_i(\tau)),
\end{eqnarray*}
where the last inequality uses the fact that $\langle x_i(\tau), y_\tau \rangle \geq 0, \forall \tau$. Now taking expectation w.r.t. the perturbation, we conclude that \footnote{There should be an expectation over $\hat{R}_i(t),$ but for simplicity, I am just writing it without the expectation. Rigorously speaking, one needs to establish a high probability bound here.}
\begin{eqnarray*}
	\hat{R}_i(t) - R_i(t) \leq \epsilon \hat{R}_i(t),
\end{eqnarray*}  
which implies that $R_i(t) \geq (1-\epsilon) R_i(t).$
Thus the regret for the original requests for logarithmic utility function is bounded by:
\begin{eqnarray} \label{regret-ub}
	\textrm{Regret}_T \leq 2 \log (1+\epsilon)T + \hat{\textrm{Regret}_T} \leq 2 \epsilon T + O\bigg( \big(\frac{N}{k\epsilon} \big)^{3/2} J\big(\frac{\epsilon k T}{N}\big) \bigg).
\end{eqnarray}
Finally, we can minimize the regret upper-bound \eqref{regret-ub} by optimizing over the perturbation probability $\epsilon.$ As an example, for the logarithmic fairness function, the optimal values are given as follows:
\begin{eqnarray*}
	\epsilon^*_{\textrm{logarithmic}} = \Omega(T^{-1/4}), ~~ \textrm{Regret}_T = O(T^{3/4}).
\end{eqnarray*}
The regret for $\alpha$-fair utility can also be optimized using a similar approach.
%In the case of $\alpha$-fair utility functions, the optimal values are given as follows:
%\begin{eqnarray*}
%	\epsilon^*_{\alpha-\textrm{fair}} = \Omega(T^{\frac{1-2\alpha}{2(1+\alpha)}}), ~~ \textrm{Regret}_T = O(T^{\frac{3}{2(1+\alpha)}}).
%\end{eqnarray*}
Strictly speaking, one needs to know the value of the functional $J_\phi(\cdot)$ to tune the optimal value of $\epsilon.$
\fi

\section{Future Directions}
\begin{enumerate}
	\item Proving tight lower bounds on regret
	\item Using predictions for the next file requests to reduce the regret bound
	\item Designing policies with small dynamic regret
	\item RL formulations
\end{enumerate}

%Interestingly, the policy $\pi$ would also simultaneously yield sublinear regret for the maxmin fairness function.
%\begin{framed}
%\textbf{Question:} Can we use \textsc{Hedge} as a meta-policy to design the policy $\pi$?
%\end{framed}
%
%\subsection{Policy design with Blackwell's approachability}
%We now use Blackwell's approachability \citep{cesa2006prediction} for designing an online learning policy that guarantees the uniform regret bound \eqref{reg-expr1} in the regime $m \leq C$ \footnote{Provide a counter-example showing that achieving sublinear regret is impossible in the regime $m>C.$} 

%Thus the causal OCO policy \eqref{olo-red}, with $w_i(t) \propto \frac{1}{R_i(t)},$ yields $\tilde{O}({\sqrt{T}})$ regret for the fair caching problem. 
%
%A better estimate may be found directly using Eqn.\ \eqref{func-ineq1}. We may write:
%\begin{eqnarray*}
%	\beta \sum_i \frac{1}{R_i(t)} \leq \frac{1}{t}\sum_i \log R_i(t) + O(\frac{1}{\sqrt{t}}) \leq m \frac{\log T}{t} + O(\frac{1}{\sqrt{t}}).
%\end{eqnarray*}
%Summing up both sides over all rounds, we have the bound:
%\begin{eqnarray*}
%	\beta \sum_{t=1}^T \sum_i\frac{1}{R_i(t)} \leq m \log^2(T) + O(\sqrt{T}).
%\end{eqnarray*}
%The last $O(\sqrt{T})$ can be reduced to $O(1/\sqrt{T}).$

%\subsection{An Online Learning Policy that guarantees the uniform regret bound \eqref{reg-expr1}}
%To show that there does exist an (albeit inefficient) online learning policy that guarantees the uniform regret bound \eqref{reg-expr1}, consider an instance of Learning with Experts advice problem as described below. 
%
%We define a collection of $P=m\binom{N}{k}$ experts such that to each user $i \in [m]$ and each subset files $y \in \binom{[N]}{k},$ we associate a corresponding ``Expert" $\mathcal{E}_{i,y}.$ The reward of the expert $(i,y)$ on round $t$ is defined as $r_{i,y} = \langle x_i(t), y \rangle.$ Then, upon running any no-regret policy (\emph{e.g.,} \textsc{Hedge}) on this instance of experts, we have the following guarantee
%\begin{eqnarray*}
%	\sum_{\tau=1}^{t} \langle x_i(\tau), y_\tau \rangle  \geq \max_{i,y} \sum_{\tau=1}^t \langle x_i(\tau), y \rangle - O(\sqrt{t}),
%\end{eqnarray*} 
%which implies \eqref{reg-expr1}. In our problem, if the expert $(i,c)$ is sampled at time $t$, the online policy simply caches the subset of files given by $c$. For the single user case $m=1$, it is known from \citet{mukhopadhyay2022k} that the \textsc{Hedge} policy can be run in almost linear time. 
%
%\subsection{Derivation of a no-regret Online Caching Policy}
%
%We seek an online caching policy $\pi$ such that for all $y^* \in \Delta^N_k,$ it guarantees
%\begin{eqnarray*}
%	\max_{i} \sum_{\tau \leq t} \langle x_i(\tau), y^*-y_\tau \rangle = O(\sqrt{t}).
%\end{eqnarray*}
%Define $g_t^i(y) \equiv \langle x_i(t), y\rangle.$ We first consider a non-causal policy $\tilde{\pi}$ that has access to the reward functions $g^i_t$'s at the beginning of round $t$. Specifically, the action of the policy $\tilde{\pi}$ at round $t$ is given by:
%\begin{eqnarray*}
%	\tilde{y}_{t+1} = \arg \max_{y \in \Delta^N_k} \min_i \sum_{\tau=1}^t g^i_\tau(y) = \arg \max_{y \in \Delta^N_k} \sum_{\tau =1}^t g_\tau^{\tilde{i}_{t+1}}(y),
%\end{eqnarray*}  
%where $\tilde{i}_{t+1}$ be the index of a user which achieves the minimum user index in the above (ties are broken arbitrarily).   
%Now consider a standard OCO problem where the reward function at round $t$ is defined as: 
%\[f_t(y)= g^{\tilde{i}_{t+1}}_t(y).\]  
%Applying the BTL lemma to the sequence of reward functions $\{f_t\}_{t=1}^T$'s we immediately conclude that, the policy $\tilde{\pi}$ has a non-positive regret, \emph{i.e.,} for all $y^* \in \Delta^N_k,$ we have that
%\begin{eqnarray*}
%	\sum_{t=1}^T f_t(y^*)- f_t(\tilde{y}_{t+1}) \leq 0.
%\end{eqnarray*} 
%The above implies that: 
%


















